On the Convergence of Black-Box Variational Inference

We provide the first convergence guarantee for full black-box variational inference (BBVI), also known as Monte Carlo variational inference. While preliminary investigations worked on simplified versions of BBVI (e.g., bounded domain, bounded support, only optimizing for the scale, and such), our setup does not need any such algorithmic modifications. Our results hold for log-smooth posterior densities with and without strong log-concavity and the location-scale variational family. Also, our analysis reveals that certain algorithm design choices commonly employed in practice, particularly, nonlinear parameterizations of the scale of the variational approximation, can result in suboptimal convergence rates. Fortunately, running BBVI with proximal stochastic gradient descent fixes these limitations, and thus achieves the strongest known convergence rate guarantees. We evaluate this theoretical insight by comparing proximal SGD against other standard implementations of BBVI on large-scale Bayesian inference problems.

==> figures/group_quadratic_narrow.tex <==

      \addplot [very thick, color=cherry3] coordinates {
(0.0001, 1100)
(0.00012195704601594415, 952)
(0.00014873521072935117, 783)
(0.00018139306939110632, 643)
(0.0002212216291070448, 527)
(0.0002697953640072999, 433)
(0.00032903445623126676, 357)
(0.0004012807031942776, 292)
(0.0004893900918477494, 241)
(0.000596845699512231, 196)
(0.0007278953843983154, 162)
(0.0008877197088985861, 133)
(0.001082636733874054, 110)
(0.0013203517797162948, 91)
(0.0016102620275609393, 74)
(0.00196382800192977, 64)
(0.002395026619987486, 53)
(0.00292090371703225, 44)
(0.003562247890262444, 37)
(0.004344412298729364, 33)
(0.005298316906283708, 29)
(0.006461670787466969, 27)
(0.007880462815669913, 29)
(0.009610779662375923, 73)
(0.0117210229753348, 1100)
(0.014294613383568447, 1100)
(0.017433288221999882, 1100)
(0.021261123338996567, 1100)
(0.02592943797404667, 1100)
(0.03162277660168379, 1100)
        };
%
      \addplot [very thick, color=cherry6] coordinates {
(0.0001, 1100)
(0.00012195704601594415, 952)
(0.00014873521072935117, 783)
(0.00018139306939110632, 642)
(0.0002212216291070448, 526)
(0.0002697953640072999, 432)
(0.00032903445623126676, 355)
(0.0004012807031942776, 291)
(0.0004893900918477494, 240)
(0.000596845699512231, 196)
(0.0007278953843983154, 162)
(0.0008877197088985861, 134)
(0.001082636733874054, 112)
(0.0013203517797162948, 95)
(0.0016102620275609393, 82)
(0.00196382800192977, 72)
(0.002395026619987486, 64)
(0.00292090371703225, 57)
(0.003562247890262444, 52)
(0.004344412298729364, 48)
(0.005298316906283708, 42)
(0.006461670787466969, 42)
(0.007880462815669913, 73)
(0.009610779662375923, 1100)
(0.0117210229753348, 1100)
(0.014294613383568447, 1100)
(0.017433288221999882, 1100)
(0.021261123338996567, 1100)
(0.02592943797404667, 1100)
(0.03162277660168379, 1100)
        };
%      
      \addplot [very thick, color=cherry1] coordinates {
(0.0001, 1100)
(0.00012195704601594415, 1100)
(0.00014873521072935117, 1100)
(0.00018139306939110632, 1100)
(0.0002212216291070448, 1100)
(0.0002697953640072999, 1100)
(0.00032903445623126676, 1100)
(0.0004012807031942776, 1100)
(0.0004893900918477494, 1100)
(0.000596845699512231, 1100)
(0.0007278953843983154, 1100)
(0.0008877197088985861, 1100)
(0.001082636733874054, 1100)
(0.0013203517797162948, 1100)
(0.0016102620275609393, 1100)
(0.00196382800192977, 1100)
(0.002395026619987486, 1100)
(0.00292090371703225, 1100)
(0.003562247890262444, 1100)
(0.004344412298729364, 1100)
(0.005298316906283708, 1033)
(0.006461670787466969, 855)
(0.007880462815669913, 698)
(0.009610779662375923, 602)
(0.0117210229753348, 697)
(0.014294613383568447, 1100)
(0.017433288221999882, 1100)
(0.021261123338996567, 1100)
(0.02592943797404667, 1100)
(0.03162277660168379, 1100)
        };

      % \addplot[very thick, black, dotted]  coordinates {
      %   (0.0003846153846153846,10)
      %   (0.0003846153846153846,1000)
      % } node[pos=0.17, left] {};


==> figures/group_quadratic_unit.tex <==

      \addplot [very thick, color=cherry3] coordinates {
        (0.0001, 1100)
        (0.00012195704601594415, 965)
        (0.00014873521072935117, 794)
        (0.00018139306939110632, 654)
        (0.0002212216291070448, 536)
        (0.0002697953640072999, 439)
        (0.00032903445623126676, 362)
        (0.0004012807031942776, 297)
        (0.0004893900918477494, 244)
        (0.000596845699512231, 199)
        (0.0007278953843983154, 164)
        (0.0008877197088985861, 135)
        (0.001082636733874054, 111)
        (0.0013203517797162948, 93)
        (0.0016102620275609393, 77)
        (0.00196382800192977, 64)
        (0.002395026619987486, 53)
        (0.00292090371703225, 45)
        (0.003562247890262444, 37)
        (0.004344412298729364, 33)
        (0.005298316906283708, 29)
        (0.006461670787466969, 27)
        (0.007880462815669913, 29)
        (0.009610779662375923, 73)
        (0.0117210229753348, 1100)
        (0.014294613383568447, 1100)
        (0.017433288221999882, 1100)
        (0.021261123338996567, 1100)
        (0.02592943797404667, 1100)
        (0.03162277660168379, 1100)
        };
      \addlegendentry{\footnotesize Proximal SGD \(\phi(x)=x\)}
%
      \addplot [very thick, color=cherry6] coordinates {
        (0.0001, 1100)
        (0.00012195704601594415, 965)
        (0.00014873521072935117, 794)
        (0.00018139306939110632, 654)
        (0.0002212216291070448, 536)
        (0.0002697953640072999, 439)
        (0.00032903445623126676, 362)
        (0.0004012807031942776, 297)
        (0.0004893900918477494, 244)
        (0.000596845699512231, 199)
        (0.0007278953843983154, 164)
        (0.0008877197088985861, 135)
        (0.001082636733874054, 111)
        (0.0013203517797162948, 93)
        (0.0016102620275609393, 77)
        (0.00196382800192977, 64)
        (0.002395026619987486, 53)
        (0.00292090371703225, 45)
        (0.003562247890262444, 37)
        (0.004344412298729364, 33)
        (0.005298316906283708, 29)
        (0.006461670787466969, 29)
        (0.007880462815669913, 58)
        (0.009610779662375923, 1100)
        (0.0117210229753348, 1100)
        (0.014294613383568447, 1100)
        (0.017433288221999882, 1100)
        (0.021261123338996567, 1100)
        (0.02592943797404667, 1100)
        (0.03162277660168379, 1100)
        };
      \addlegendentry{\footnotesize SGD \(\phi(x)=x\)}
      %
      \addplot [very thick, color=cherry1] coordinates {
        (0.0001, 1100)
        (0.00012195704601594415, 1100)
        (0.00014873521072935117, 1100)
        (0.00018139306939110632, 1100)
        (0.0002212216291070448, 1100)
        (0.0002697953640072999, 1100)
        (0.00032903445623126676, 1100)
        (0.0004012807031942776, 1100)
        (0.0004893900918477494, 1100)
        (0.000596845699512231, 987)
        (0.0007278953843983154, 811)
        (0.0008877197088985861, 674)
        (0.001082636733874054, 554)
        (0.0013203517797162948, 467)
        (0.0016102620275609393, 388)
        (0.00196382800192977, 322)
        (0.002395026619987486, 267)
        (0.00292090371703225, 222)
        (0.003562247890262444, 186)
        (0.004344412298729364, 162)
        (0.005298316906283708, 131)
        (0.006461670787466969, 124)
        (0.007880462815669913, 129)
        (0.009610779662375923, 133)
        (0.0117210229753348, 306)
        (0.014294613383568447, 1100)
        (0.017433288221999882, 1100)
        (0.021261123338996567, 1100)
        (0.02592943797404667, 1100)
        (0.03162277660168379, 1100)
        };
      \addlegendentry{\footnotesize SGD \(\phi(x) = \mathrm{softplus}(x)\) }


      % \addplot[very thick, black, dotted]  coordinates {
      %   (0.0003846153846153846,10)
      %   (0.0003846153846153846,1000)
      % } node[pos=0.17, left] {};


==> figures/group_quadratic_verynarrow.tex <==

      \addplot [very thick, color=cherry3] coordinates {
        (0.0001, 1100)
        (0.00012195704601594415, 952)
        (0.00014873521072935117, 783)
        (0.00018139306939110632, 643)
        (0.0002212216291070448, 527)
        (0.0002697953640072999, 433)
        (0.00032903445623126676, 357)
        (0.0004012807031942776, 292)
        (0.0004893900918477494, 241)
        (0.000596845699512231, 196)
        (0.0007278953843983154, 162)
        (0.0008877197088985861, 133)
        (0.001082636733874054, 110)
        (0.0013203517797162948, 91)
        (0.0016102620275609393, 74)
        (0.00196382800192977, 64)
        (0.002395026619987486, 53)
        (0.00292090371703225, 44)
        (0.003562247890262444, 37)
        (0.004344412298729364, 33)
        (0.005298316906283708, 29)
        (0.006461670787466969, 27)
        (0.007880462815669913, 29)
        (0.009610779662375923, 73)
        (0.0117210229753348, 1100)
        (0.014294613383568447, 1100)
        (0.017433288221999882, 1100)
        (0.021261123338996567, 1100)
        (0.02592943797404667, 1100)
        (0.03162277660168379, 1100)
        };
%
      \addplot [very thick, color=cherry6] coordinates {
        (0.0001, 1100)
        (0.00012195704601594415, 1100)
        (0.00014873521072935117, 1100)
        (0.00018139306939110632, 1100)
        (0.0002212216291070448, 1100)
        (0.0002697953640072999, 1100)
        (0.00032903445623126676, 1057)
        (0.0004012807031942776, 915)
        (0.0004893900918477494, 789)
        (0.000596845699512231, 680)
        (0.0007278953843983154, 588)
        (0.0008877197088985861, 500)
        (0.001082636733874054, 429)
        (0.0013203517797162948, 367)
        (0.0016102620275609393, 315)
        (0.00196382800192977, 267)
        (0.002395026619987486, 228)
        (0.00292090371703225, 194)
        (0.003562247890262444, 164)
        (0.004344412298729364, 140)
        (0.005298316906283708, 123)
        (0.006461670787466969, 104)
        (0.007880462815669913, 95)
        (0.009610779662375923, 1100)
        (0.0117210229753348, 1100)
        (0.014294613383568447, 1100)
        (0.017433288221999882, 1100)
        (0.021261123338996567, 1100)
        (0.02592943797404667, 1100)
        (0.03162277660168379, 1100)
        };
%      
      \addplot [very thick, color=cherry1] coordinates {
        (0.0001, 1100)
        (0.00012195704601594415, 1100)
        (0.00014873521072935117, 1100)
        (0.00018139306939110632, 1100)
        (0.0002212216291070448, 1100)
        (0.0002697953640072999, 1100)
        (0.00032903445623126676, 1100)
        (0.0004012807031942776, 1100)
        (0.0004893900918477494, 1100)
        (0.000596845699512231, 1100)
        (0.0007278953843983154, 1100)
        (0.0008877197088985861, 1100)
        (0.001082636733874054, 1100)
        (0.0013203517797162948, 1100)
        (0.0016102620275609393, 1100)
        (0.00196382800192977, 1100)
        (0.002395026619987486, 1100)
        (0.00292090371703225, 1100)
        (0.003562247890262444, 1100)
        (0.004344412298729364, 1100)
        (0.005298316906283708, 1100)
        (0.006461670787466969, 1100)
        (0.007880462815669913, 1100)
        (0.009610779662375923, 1069)
        (0.0117210229753348, 1035)
        (0.014294613383568447, 1100)
        (0.017433288221999882, 1100)
        (0.021261123338996567, 1100)
        (0.02592943797404667, 1100)
        (0.03162277660168379, 1100)
        };

      % \addplot[very thick, black, dotted]  coordinates {
      %   (0.0003846153846153846,10)
      %   (0.0003846153846153846,1000)
      % } node[pos=0.17, left] {};


==> main-pratendconvexity.tex <==


\prAtEndRestateix*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndix}The special case \textbf {(i)} is proven by \citet [Theorem 9]{domke_provable_2020}. We focus on the general statement \textbf {(ii)}. \par If \(\ell \) is \(\mu \)-strongly convex, the inequality \begin {align} \ell \left (\vz \right ) - \ell \left (\vz '\right ) \geq \inner { \nabla \ell \left (\vz '\right ) }{ \vz -\vz ^{\prime } } + \frac {\mu }{2} \norm {\vz - \vz ^{\prime }}_2^2 \label {eq:log_concave_strong_convexity_inequality} \end {align} holds, where the general convex case is obtained as a special case with \(\mu = 0\). The goal is to relate this to the (\(\mu \)-strong-)convexity of the energy with respect to the variational parameters given by \begin {align*} f\left ( \vlambda \right ) - f\left ( \vlambda ' \right ) \geq \inner { \nabla _{\vlambda } f\left ( \vlambda ^{\prime } \right ) }{ \vlambda - \vlambda ^{\prime } } + \frac {\mu }{2} \norm { \vlambda - \vlambda ^{\prime } }_2^2. \nonumber \end {align*} \par \paragraph {Proof of (ii)} Plugging the reparameterized latent variables to \cref {eq:log_concave_strong_convexity_inequality} and taking the expectation, we have \begin {alignat*}{2} & & \mathbb {E} \ell \left ( \mathcal {T}_{\vlambda }\left (\rvvu \right ) \right ) - \mathbb {E} \ell \left ( \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) \right ) &\geq \mathbb {E} \inner { \nabla \ell \left ( \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right )\right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) } + \frac {\mu }{2} \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2 \\ &\Leftrightarrow \qquad & f\left (\vlambda \right ) - f\left (\vlambda ^{\prime }\right ) &\geq \mathbb {E} \inner { \nabla \ell \left ( \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right )\right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) } + \frac {\mu }{2} \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2 \\ &\Leftrightarrow \qquad & f\left (\vlambda \right ) - f\left (\vlambda ^{\prime }\right ) &\geq \mathbb {E} \inner { \nabla g\left ( \vlambda ^{\prime }; \rvvu \right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) } + \frac {\mu }{2} \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2 \end {alignat*} Thus, the energy is convex if and only if \begin {align*} \mathbb {E} \inner { g \left ( \vlambda ; \rvvu \right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) } \geq \inner { \nabla f\left (\vlambda \right ) }{ \vlambda - \vlambda ^{\prime } } \end {align*} holds. This is established by \cref {thm:innerproduct_z_t}. \par \paragraph {Proof of (iii)} We now prove that, under the nonlinear parameterization, the energy cannot be strongly convex. When the energy is convex, it is also strongly convex if and only if \[ \frac {\mu }{2} \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2 \geq \frac {\mu }{2} \norm { \vlambda - \vlambda ^{\prime } }_2^2. \] \par From the proof of \citet [Lemma 5]{domke_provable_2020}, it follows that \begin {align*} \mathbb {E} \norm {\mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right )}_2^2 &= \norm {\mC - \mC ^{\prime }}_{\mathrm {F}}^2 + \norm { \vm - \vm ^{\prime } }_2^2. \end {align*} Furthermore, under nonlinear parameterizations, \begin {align} &\norm {\mC - \mC ^{\prime }}_{\mathrm {F}}^2 + \norm { \vm - \vm ^{\prime } }_2^2 \nonumber \\ &\;= \norm { \left ( \mD _{\phi }\left (\vs \right ) - \mD _{\phi }\left (\vs ^{\prime }\right ) \right ) - \left ( \mL - \mL ^{\prime }\right ) }_{\mathrm {F}}^2 + \norm { \vm - \vm ^{\prime } }_2^2, \nonumber \shortintertext {expanding the quadratic,} &\;= \norm { \mD _{\phi }\left (\vs \right ) - \mD _{\phi }\left (\vs ^{\prime }\right ) }_{\mathrm {F}}^2 + \norm { \mL - \mL ^{\prime } }_{\mathrm {F}}^2 - 2 \inner { \mD _{\phi }\left (\vs \right ) - \mD _{\phi }\left (\vs ^{\prime }\right ) }{ \mL - \mL ^{\prime } }_{\mathrm {F}} + \norm { \vm - \vm ^{\prime } }_2^2, \nonumber \shortintertext {and since \(\mD _{\phi }\left (\vs \right )\) and \(\mL \) reside in different sub-spaces, they are orthogonal. Thus,} &\;= \norm { \mD _{\phi }\left (\vs \right ) - \mD _{\phi }\left (\vs ^{\prime }\right ) }_{\mathrm {F}}^2 + \norm { \mL - \mL ^{\prime } }_{\mathrm {F}}^2 + \norm { \vm - \vm ^{\prime } }_2^2 \nonumber \\ &\;= \norm { \phi \left (\vs \right ) - \phi \left (\vs ^{\prime }\right ) }_{2}^2 + \norm { \mL - \mL ^{\prime } }_{\mathrm {F}}^2 + \norm { \vm - \vm ^{\prime } }_2^2. \label {eq:thm_energy_log_concave_eq1} \end {align} For the energy term to be strongly convex, \cref {eq:thm_energy_log_concave_eq1} must be bounded \textit {below} by \(\norm {\vlambda - \vlambda ^{\prime }}_2^2\). Evidently, this implies that a necessary and sufficient condition is that \[ \abs { \phi \left (s_{ii}\right ) - \phi \left (s_{ii}^{\prime }\right ) } \geq L \, \abs { s_{ii} - s_{ii}^{\prime } } \] by some constant \(0 < L < \infty \). Notice that the direction of the inequality is reversed from the Lipschitz condition. Unfortunately, there is no such continuous and differentiable function \(\phi : \mathbb {R} \rightarrow \mathbb {R}_+\), as established by \cref {thm:L_does_not_exist}. Thus, for any diagonal conditioner \(\phi \in \mathrm {C}^1\left (\mathbb {R}, \mathbb {R}_+\right )\), the energy cannot be strongly convex.\end{proof}


==> main-pratendconvexityanalysis.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateviii}\label{thm:prAtEndviii}\label {thm:L_does_not_exist} For any function $f \in \mathrm {C}^1(\mathbb {R}, \mathbb {R}_+)$ , there is no constant \(0 < L < \infty \) such that \[ \abs { f(x) - f(y) } \geq L \abs {x - y}. \]\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndviii}\par \par \par \par \par \par Suppose for the sake of contradiction that such $L > 0$ exists. Letting $y \to x$ gives $\abs {f^\prime (x)} \geq L$ for all $x \in \mathbb {R}$. For each $x$, either $f^\prime (x) \leq -L$ or $f^\prime (x) \geq L$ holds. We discuss two cases based on the value of $f^\prime (0)$. \par If $f^\prime (0) \geq L$, we claim that $f^\prime (x) \geq L$ for all $x \in \mathbb {R}$. Otherwise, $f^\prime (x) < L$ for some $x$ implies $f^\prime (x) \leq - L$. By the intermediate value theorem ($f^\prime $ is continuous), there exists a point $y$ between $0$ and $x$ that attains the value $f^\prime (y) = 0$, which is a contradiction. \par Now that $f^\prime (x) \geq L > 0$ for all $x$, $f$ is an increasing function. For any $x < 0$, we have \begin {align*} f(x) & = f(x) - f(0) + f(0) \\ & = - \abs {f(x) - f(0)} + f(0) \\ & \leq - L \abs {x} + f(0). \end {align*} Here, we can plug \(x^{\prime } = - \frac {f(0)}{L}\) as \[ f(x^{\prime }) = - L \abs {- \frac {f(0)}{L}} + f(0) = - \abs {f(0) } + f(0) \leq 0, \] which implies that \(f(x^{\prime }) \notin \mathbb {R}_+\), which is a contradiction. \par Now we discuss the second case $f^\prime (0) \leq -L$. By a similar argument, $f^\prime (x) \leq -L$ for all $x \in \mathbb {R}$. Thus, $f$ is a decreasing function. For any $x > 0$, we have \begin {align*} f(x) & = f(x) - f(0) + f(0) \\ & = - \abs {f(x) - f(0)} + f(0) \\ & \leq - L x + f(0). \end {align*} Picking $x^\prime = \frac {f(0)}{L}$ results in $f(x^\prime ) \notin \mathbb {R}_+$, which is a contradiction.\end{proof}


==> main-pratendconvexitylemma.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatevii}\label{thm:prAtEndvii}\label {thm:innerproduct_z_t} Let \(\ell \) be convex. Then, for a convex nonlinear \(\phi \), the inequality \[ \inner { \nabla _{\vlambda } f\left (\vlambda \right ) }{ \vlambda - \vlambda ^{\prime } } \leq \mathbb {E} \inner { \nabla g\left (\vlambda ; \rvvu \right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) } \] holds for all \(\vlambda \in \Lambda \) if and only if \cref {assumption:peculiar_convexity} holds. For the linear parameterization, the inequality becomes equality.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvii}First, notice that the left-hand side is \begin {align} &\inner { \nabla _{\vlambda } f\left (\vlambda \right ) }{ \vlambda - \vlambda ^{\prime } } \nonumber = \sum _{i = 1}^p \inner { \nabla _{\vlambda } \mathbb {E} \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) }{ \vlambda - \vlambda ^{\prime } } \nonumber = \mathbb {E} \sum _{i = 1}^p \inner { { \left ( \frac { \partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda _i} \right ) } g\left ( \vlambda ; \rvvu \right ) }{ \vlambda - \vlambda ^{\prime } }. \nonumber \shortintertext {By restricting us to the location-scale family, we then get} &= \mathbb {E}\, \Bigg ( \underbrace { \sum _{i} {\left ( \frac { \partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial m_i} \right ) } \, g\left ( \vlambda ; \rvvu \right ) {\left ( m_i - m^{\prime }_i \right )} }_{\text {convexity with respect to \(\vm \)}} + \underbrace { \sum _{ij} { \left ( \frac { \partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial L_{ij}} \right ) } \, g\left ( \vlambda ; \rvvu \right ) \left ( L_{ij} - L^{\prime }_{ij} \right ) }_{\text {convexity with respect to \(\mL \)}} \nonumber \\ &\qquad + \underbrace { \sum _{i} \mathbb {E} \left ( \frac { \partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial s_{i}} \right ) \, g\left ( \vlambda ; \rvvu \right ) {\left ( s_{i} - s^{\prime }_{i} \right )} }_{\text {convexity with respect to \(\vs \)}} \Bigg ), \nonumber \shortintertext {and plugging the derivatives of the reparameterization function,} &= \mathbb {E}\, \Bigg ( \sum _{i} g_i\left ( \vlambda ; \rvvu \right ) \, {\left ( m_i - m^{\prime }_i \right )} + \sum _{i} \sum _{j < i} \rvu _j \, g_i\left ( \vlambda ; \rvvu \right ) \, \left ( L_{ij} - L^{\prime }_{ij} \right ) + \sum _{i} \phi ^{\prime }\left (s_{i}\right ) \rvu _i \, g_i\left ( \vlambda ; \rvvu \right ) \, \left ( s_{i} - s^{\prime }_{i} \right ) \Bigg ). \nonumber \end {align} \par On the other hand, the right-hand side follows as \begin {align*} &\mathbb {E}\, \big \langle { \nabla g\left ( \vlambda ; \rvvu \right ),\; \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) \big \rangle } \nonumber \\ &\;= \mathbb {E}\, \bigg ( \big \langle { g\left ( \vlambda ; \rvvu \right ),\; }{ \vm - \vm ^{\prime } \big \rangle } \, + \big \langle { g\left ( \vlambda ; \rvvu \right ),\; }{ \left ( \mL - \mL ^{\prime } \right ) \rvvu \big \rangle } + \big \langle { g\left ( \vlambda ; \rvvu \right ),\; \left ( \mPhi \left ( \vs \right ) - \mPhi \left ( \vs ^{\prime } \right ) \right ) \rvvu \big \rangle } \bigg ) \\ &\;=\mathbb {E}\, \Bigg ( \sum _{i} g_i\left ( \vlambda ; \rvvu \right ) \, {\left ( m_i - m^{\prime }_i \right )} + \sum _{i} \sum _{j < i} \rvu _j g_i\left ( \vlambda ; \rvvu \right ) \, \left ( L_{ij} - L^{\prime }_{ij} \right ) + \sum _{i} g_i\left ( \vlambda ; \rvvu \right ) \, \rvu _i \left ( \phi \left ( s_{i} \right ) - \phi \left ( s^{\prime }_{i} \right ) \right ) \Bigg ). \end {align*} The convexity with respect to the \(\vm \) and \(\mL \) is clear from the first two terms; they are equal. The statement is now up to the last term. That is, the statement holds if \begin {equation} \mathbb {E} \sum _{i} g_i\left ( \vlambda ; \rvvu \right ) \, \rvu _i \, \phi ^{\prime }\left (s_{i}\right ) \left ( s_{i} - s^{\prime }_{i} \right ) \;\leq \; \mathbb {E} \sum _{i} g_i\left ( \vlambda ; \rvvu \right ) \, \rvu _i \left ( \phi \left ( s_{i} \right ) - \phi \left ( s^{\prime }_{i} \right ) \right ). \label {eq:innerproduct_z_to_t} \end {equation} For this, we will show that \cref {assumption:peculiar_convexity} is both necessary and sufficient. \par \paragraph {Proof of sufficiency} \cref {eq:innerproduct_z_to_t} holds if \[ \mathbb {E} g_i\left ( \vlambda ; \rvvu \right ) \, \rvu _i \geq 0 \] for all \(i = 1, \ldots , d\), which is non other than \cref {assumption:peculiar_convexity}. \par \paragraph {Proof of necessity} Suppose that the inequality \[ \inner { \nabla _{\vlambda } f\left (\vlambda \right ) }{ \vlambda - \vlambda ^{\prime } } \leq \mathbb {E} \inner { g\left (\vlambda ; \rvvu \right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) } \] holds for all \(\vlambda \in \Lambda \), implying \[ \sum _i \mathbb {E} \, \rvu _i g_i\left ( \vlambda ; \rvvu \right ) \phi '(s_{i}) (s_{i} - s'_{i}) \le \sum _i \mathbb {E} \, \rvu _i g_i\left ( \vlambda ; \rvvu \right ) \big ( (\phi (s_{i})-\phi (s'_{i}) \big ). \] \par For any \(\vlambda \), we are free to set any \(\vlambda ' \in \Lambda \) and check whether we can retrieve \cref {assumption:peculiar_convexity} for this specific \(\vlambda \). Now, for each axis $i$, set $s_{j}' = s_{j}$ for all $j\neq i$, then \[ \mathbb {E} \, \rvu _i \, g_i\left ( \vlambda ; \rvvu \right ) \phi '(s_{i}) (s_{i} - s'_{i}) \le \mathbb {E} \, \rvu _i \, g_i\left ( \vlambda ; \rvvu \right ) \left (\phi (s_{i}) - \phi (s'_{i}) \right ). \] Since \(\phi \) is assumed to be convex such that \begin {align*} \phi ^{\prime }\left (s_{i}\right ) \left ( s_{i} - s^{\prime }_{i} \right ) \leq \phi \left (s_{i}\right ) - \phi \left (s_{i}^{\prime }\right ). \end {align*} it follows that \begin {align} \mathbb {E} \, \rvu _i \, g_i\left ( \vlambda ; \rvvu \right ) \geq 0. \end {align} Therefore, for any \(\vlambda \in \Lambda \) it must be that \cref {assumption:peculiar_convexity} holds.\end{proof}

\prAtEndRestatex*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndx}For \textbf {(i)}, the key property is the monotonicity of the gradient. \paragraph {Proof of (i)} For the mean-field family, recall that \[ C_{ii} = \phi \left (s_i\right ). \] Also, observe that \[ \mC \rvvu + \vm = (C_{11} \rvu _1 + m_1, \ldots , C_{dd} \rvu _d + m_d). \] By the property of convex functions, \(\nabla \ell \) is monotone such that \[ \inner { \nabla \ell \left (\vz \right ) - \nabla \ell \left (\vz ^{\prime }\right ) }{ \vz - \vz ^{\prime } } \geq 0. \] Now, by setting $\rvvz = \mC \rvvu + \vm $ and $\rvvz ' = \mC \rvvu + \vm - C_{ii} \rvu _i \boldupright {e}_i$, we obtain \[ \inner { \nabla \ell \left ( \mC \rvvu + \vm \right ) - \nabla \ell \left ( \mC \rvvu + \vm - C_{ii} \rvu _i \boldupright {e}_i \right ) }{ C_{ii} \rvu _i \boldupright {e}_i } \geq 0 \] for every \(i = 1, \ldots , d\). \par For the mean-field family, \(\mC \rvvu + \vm - C_{ii} \rvu _i \boldupright {e}_i\) is now independent of \(\rvu _i\). Thus, \begin {align*} \mathbb {E}\, C_{ii} \rvu _i \mathrm {D}_i \ell \left (\mC \rvvu + \vm \right ) &\geq \mathbb {E}\, C_{ii} \rvu _i \, \mathrm {D}_i \ell \left (\mC \rvvu + \vm - \boldupright {e}_i C_{ii} \rvu _i \right ) \\ &= C_{ii} \left ( \mathbb {E}\, \rvu _i \right ) \left ( \mathbb {E} \, \mathrm {D}_i f \left (\mC \rvvu + \vm - \boldupright {e}_i C_{ii} \rvu _i \right ) \right ) \\ &= 0, \end {align*} where \(\mathrm {D}_i f\) denotes the \(i\)th axis of \(\nabla f\). Since \(C_{ii} > 0\) by design, \[ \mathbb {E}\, C_{ii} \rvu _i \mathrm {D}_i f \left (\mC \rvvu + \vm \right ) > 0 \quad \Leftrightarrow \quad \mathbb {E}\, \rvu _i \mathrm {D}_i f \left (\mC \rvvu + \vm \right ) > 0, \] which is \cref {assumption:peculiar_convexity}. \par \paragraph {Proof of (ii)} We provide an example that proves the statement. Let \(\ell (\vz ) = \frac {1}{2} \vz ^{\top } \mA \vz \). Then, \begin {align*} g\left (\vlambda ; \rvvu \right ) = \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) = \mA \left ( \mC \rvvu + \vm \right ) = \mA \mC \rvvu + \mA \vm . \end {align*} Suppose that we choose \(\vlambda \) such that \[ \mC = \begin {bmatrix} 1 & 0 \\ 1 & 1 \end {bmatrix} \] and \(\vm = \boldupright {0}\). Also, setting \[ \mA = \begin {bmatrix} 1 & -2 \\ -2 & 5 \end {bmatrix}, \] we get a strongly convex function \(\ell \). Then, \begin {align*} g\left (\vlambda ; \rvvu \right ) = \mA \mC \rvvu = \begin {bmatrix} 1 & -2 \\ -2 & 5 \end {bmatrix} \begin {bmatrix} 1 & 0 \\ 1 & 1 \end {bmatrix} \begin {bmatrix} \rvu _1 \\ \rvu _2 \end {bmatrix} = \begin {bmatrix} -1 & -2 \\ 3 & 5 \end {bmatrix} \begin {bmatrix} \rvu _1 \\ \rvu _2 \end {bmatrix} = \begin {bmatrix} -\rvu _1 - 2 \rvu _2 \\ 3 \rvu _1 + 5 \rvu _2 \end {bmatrix} \end {align*} Finally, we have \begin {align*} \mathbb {E} g_1\left (\vlambda ; \rvvu \right ) \rvu _1 &= \mathbb {E}\left ( -\rvu _1 - 2 \rvu _2 \right ) \rvu _1 = -1 < 0, \end {align*} which violates \cref {assumption:peculiar_convexity}.\end{proof}


==> main-pratendexamplesmoothness.tex <==


\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndvi}Since the gradient is \[ \nabla \ell \left (\vz \right ) = \mA \vz , \] combined with reparameterization, we have \begin {align*} g\left (\vlambda ; \rvvu \right ) = \mA \left ( \mC \rvvu + \vm \right ) \end {align*} Then, for each coordinate \(i = 1, \ldots , d\), we have \begin {align*} \mathbb {E}g_i\left (\vlambda ; \rvvu \right ) \rvu _i \phi ''(s_i) &= \mathbb {E} \left ( \sum _{j} \sum _{k \leq j} A_{ij} C_{jk} \rvu _{k} + \sum _{j} A_{ij} m_{j} \right ) \rvu _i \phi ''(s_i) \\ &= \sum _{j} \sum _{k \leq j} A_{ij} C_{jk} \mathbb {E} \rvu _{k} \rvu _i \phi ''(s_i) + \sum _{j} A_{ij} m_{j} \mathbb {E} \rvu _i \phi ''(s_i), \shortintertext {and from \cref {assumption:symmetric_standard},} &= \phi ''(s_i) \sum _{j} \sum _{k \leq j} A_{ij} C_{jk} \mathbb {1}_{k=i} \\ &= \phi ''(s_i) \sum _{j} A_{ij} C_{ji}. \end {align*} Furthermore, the diagonal of \(\mC \) involves \(\phi \) such that \begin {align*} \mathbb {E}g_i\left (\vlambda ; \rvvu \right ) \rvu _i \phi ''(s_i) &= \underbrace {A_{ii} \phi \left (s_i\right ) \phi ''\left (s_i\right )}_{T_{\mathrm {diag}}} + \underbrace { \sum _{j < i} A_{ij} C_{ji} \phi ''(s_i) }_{T_{\mathrm {off}}}. \end {align*} \par For the softplus function, we have \[ 0 < \phi ''\left (s\right ) < 1 \] for any finite \(s\), and we have \[ \sup _{s} \phi \left (s\right ) \phi ^{\prime \prime }\left (s\right ) \approx 0.26034, \] where the supremum was numerically approximated. Then, it is clear that \(T_{\mathrm {diag}}\) is finite as long as the diagonals of \(\mA \) are finite. Furthermore, we have the following: \begin {enumerate}[label=\textbf {(\roman *)}] \item If \(\mA \) is diagonal, then \(T_{\mathrm {off}}\) is 0. \item If \(\mA \) is dense but \(\mC \) is diagonal due to the use of the mean-field family, \(T_{\mathrm {off}}\) is again 0. \item However, when both \(\mA \) and \(\mC \) are not diagonal, \(T_{\mathrm {off}}\) can be made arbitrarily large. \end {enumerate} \par \par \end{proof}


==> main-pratendexternal.tex <==


\begin{restatable}[]{lemma}{prAtEndRestatexix}\label{thm:prAtEndxix}\label {thm:linearity} Let \(\phi \left (x\right ) = x\). Then, the parameterization is linear in the sense that \(\mathcal {T}_{\vlambda }\) is a bilinear function such that \[ \mathcal {T}_{\vlambda - \vlambda ^{\prime }}\left (\vu \right ) = \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ). \] for any \(\vlambda , \vlambda ' \in \Lambda \).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxix}\begin {align*} \mathcal {T}_{\vlambda - \vlambda ^{\prime }}\left (\vu \right ) &= \left ( \mC \left (\vlambda - \vlambda ^{\prime }\right ) \right ) \vu + \left (\vm - \vm ^{\prime }\right ) \nonumber \\ &= \left ( \mD _{\phi }\left (\vs - \vs '\right ) + \left (\mL - \mL '\right ) \right ) \vu + \left (\vm - \vm ^{\prime }\right ), \nonumber \shortintertext {using the fact that \(\phi \) is the identity function,} &= \left ( \mD _{\phi }\left (\vs \right ) - \mD _{\phi }\left (\vs '\right ) + \left (\mL - \mL '\right ) \right ) \vu + \left (\vm - \vm ^{\prime }\right ) \nonumber \\ &= \left ( \mC \left (\vlambda \right ) - \mC \left (\vlambda ^{\prime }\right ) \right ) \vu + \left ( \vm + \vm ^{\prime } \right ) \nonumber \\ &= \left ( \mC \left (\vlambda \right ) \vu + \vm \right ) - \left ( \mC \left (\vlambda ^{\prime }\right ) \vu + \vm ^{\prime } \right ) \nonumber \\ &= \mathcal {T}_{\vlambda }\left (\vu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\vu \right ). \end {align*} The linearity with respect to \(\vu \) is obvious.\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexx}\label{thm:prAtEndxx}\label {thm:jacobian_reparam_inner_original} Let the linear parameterization be used. Then, for any \(\vlambda , \vlambda ' \in \Lambda \), the inner product of the Jacobian of the reparameterization function satisfies the following equalities for any \(\vu \in \mathbb {R}^d\). \begin {enumerate}[label=\textbf {(\roman *)},itemsep=-1ex] \item For the Cholesky family \citep [Lemma 8]{domke_provable_2019}, \[ {\left (\frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right ) }{ \partial \vlambda }\right )}^{\top } \frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right ) }{ \partial \vlambda } = \left ( 1 + \norm {\vu }_2^2 \right ) \boldupright {I} \] \par \item For the mean-field family~\citep [Lemma 1]{kim_practical_2023}, \[ {\left (\frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right ) }{ \partial \vlambda }\right )}^{\top } \frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right ) }{ \partial \vlambda } = \left ( 1 + {\lVert \mU ^2 \rVert }_{\mathrm {F}} \right ) \boldupright {I}, \] where \(\mU = \mathrm {diag}\left (u_1, \ldots , u_d\right )\). \end {enumerate}\end{restatable}

\begin{restatable}[]{lemma}{prAtEndRestatexxi}\label{thm:prAtEndxxi}\label {thm:u_normsquared_marginalization_original} Let the linear parameterization be used. Then, for any \(\vlambda \in \Lambda \) and any \(\vz \in \mathbb {R}^d\), the following relationships hold. \begin {enumerate}[label=\textbf {(\roman *)},itemsep=-1ex] \item For the Cholesky family~\citep [Lemma 2]{domke_provable_2019}, \[ \mathbb {E} \left ( 1 + \norm {\rvvu }_2^2 \right ) \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \vz }_2^2 = \left (d + 1\right ) \norm { \vm - \vz }_2^2 + \left (d + k_{\varphi }\right ) \norm { \mC }_{\mathrm {F}}^2 \] \item For the mean-field family~\citep [Lemma 2]{kim_practical_2023}, \[ \mathbb {E} \left ( 1 + {\lVert \rvmU ^2 \rVert }_{\mathrm {F}} \right ) \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \vz }_2^2 \leq \left ( \sqrt {d k_{\varphi }} + k_{\varphi } \sqrt {d} + 1 \right ) \norm { \vm - \vz }_2^2 + \left (2 k_{\varphi } \sqrt {d} + 1\right ) \norm { \mC }_{\mathrm {F}}^2. \] \end {enumerate}\end{restatable}

\begin{restatable}[]{corollary}{prAtEndRestatexxii}\label{thm:prAtEndxxii}\label {thm:u_normsquared_marginalization} Let the linear parameterization be used and \(\vlambda , \vlambda ^{\prime } \in \Lambda \) be any pair of variational parameters. \begin {enumerate}[label=\textbf {(\roman *)},itemsep=-1ex] \item For the Cholesky family,\label {item:thm_u_normsquared_cholesky} \[ \mathbb {E} \left ( 1 + \norm {\rvvu }_2^2 \right ) \norm {\mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) - \mathcal {T}_{\vlambda }\left (\rvvu \right ) }_2^2 \leq (k_{\varphi } + d) \norm {\vlambda - \vlambda ^{\prime }}_2^2 \] \item For the mean-field family,\label {item:thm_u_normsquared_meanfield} \[ \mathbb {E} \left ( 1 + {\lVert \rvmU ^2\rVert }_{\mathrm {F}} \right ) \norm {\mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) - \mathcal {T}_{\vlambda }\left (\rvvu \right ) }_2^2 \leq (2 k_{\varphi } \sqrt {d} + 1) \norm {\vlambda - \vlambda ^{\prime }}_2^2 \] \end {enumerate}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxxii}The results are a direct consequence of \cref {thm:u_normsquared_marginalization_original} and \cref {thm:linearity}. \paragraph {Proof of \labelcref *{item:thm_u_normsquared_cholesky}} We start from~\cref {thm:u_normsquared_marginalization_original} as \begin {align*} \mathbb {E} \left ( 1 + \norm {\rvvu }_2^2 \right ) \norm { \mathcal {T}_{\vlambda - \vlambda ^{\prime }}\left (\rvvu \right ) - \vz }_2^2 &= \left (d + 1\right ) \norm { \left ( \vm - \vm ^{\prime } \right ) - \vz }_2^2 + \left (d + k_{\varphi }\right ) \norm { \mC \left (\vlambda \right ) - \mC \left (\vlambda ^{\prime }\right ) }_{\mathrm {F}}^2, \shortintertext {setting \(\vz = \boldupright {0}\),} &= \left (d + 1\right ) \norm { \vm - \vm ^{\prime } }_2^2 + \left (d + k_{\varphi }\right ) \norm { \mC \left (\vlambda \right ) - \mC \left (\vlambda ^{\prime }\right ) }_{\mathrm {F}}^2, \shortintertext {and since \(k_{\varphi } \geq 3\) by the property of the kurtosis,} &\leq \left (d + k_{\varphi }\right ) \left ( \norm { \vm - \vm ^{\prime } }_2^2 + \norm { \mC \left (\vlambda \right ) - \mC \left (\vlambda ^{\prime }\right ) }_{\mathrm {F}}^2 \right ) \\ &= \left (d + k_{\varphi }\right ) \norm {\vlambda - \vlambda ^{\prime }}_2^2. \end {align*} \par \paragraph {Proof of \labelcref *{item:thm_u_normsquared_meanfield}} Similarly, for the mean-field family, we can apply~\cref {thm:u_normsquared_marginalization_original} as \begin {align*} \mathbb {E} \left ( 1 + {\lVert \rvmU ^2 \rVert }_{\mathrm {F}} \right ) \norm { \mathcal {T}_{\vlambda - \vlambda ^{\prime }}\left (\rvvu \right ) - \bar {\vz } }_2^2 &\leq \left ( \sqrt {d k_{\varphi }} + k_{\varphi } \sqrt {d} + 1 \right ) \norm { \left (\vm - \vm ^{\prime }\right ) - \bar {\vz } }_2^2 + \left (2 k_{\varphi } \sqrt {d} + 1\right ) \norm { \mC - \mC ^{\prime } }_{\mathrm {F}}^2, \shortintertext {setting \(\vz = \boldupright {0}\),} &= \left ( \sqrt {d k_{\varphi }} + k_{\varphi } \sqrt {d} + 1 \right ) \norm {\vm - \vm ^{\prime }}_2^2 + \left (2 k_{\varphi } \sqrt {d} + 1\right ) \norm { \mC - \mC ^{\prime } }_{\mathrm {F}}^2, \shortintertext {and since \(k_{\varphi } \geq 3\) by the property of the kurtosis,} &\leq \left ( 2 k_{\varphi } \sqrt {d} + 1 \right ) \left ( \norm { \vm - \vm ^{\prime } }_2^2 + \norm { \mC \left (\vlambda \right ) - \mC \left (\vlambda ^{\prime }\right ) }_{\mathrm {F}}^2 \right ) \\ &= \left ( 2 k_{\varphi } \sqrt {d} + 1 \right ) \norm {\vlambda - \vlambda ^{\prime }}_2^2. \end {align*}\end{proof}

\begin{restatable}[]{lemma}{prAtEndRestatexxiii}\label{thm:prAtEndxxiii}\label {thm:difference_t_z_identity} For the linear parameterization, \[ \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda '}\left (\rvvu \right ) }_2^2 = \norm { \vlambda - \vlambda ' }_2^2 \] for any \(\vlambda , \vlambda ' \in \Lambda \).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxxiii}First notice that, for linear parameterizations, we have \begin {align*} \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) }_2^2 &= \mathbb {E} \norm { \mC \rvvu + \vm }_2^2 \\ &= \mathbb {E} \rvvu ^{\top } \mC ^{\top } \mC \rvvu + \norm {\vm }_2^2 + 2 \vm ^{\top } \mC \mathbb {E} \rvvu \\ &= \mathbb {E} \operatorname {tr} \left ( \rvvu ^{\top } \mC ^{\top } \mC \rvvu \right ) + \norm {\vm }_2^2 + 2 \vm ^{\top } \mC \mathbb {E} \rvvu , \shortintertext {rotating the elements of the trace,} &= \operatorname {tr} \left ( \mC ^{\top } \mC \mathbb {E} \rvvu \rvvu ^{\top } \right ) + \norm {\vm }_2^2 + 2 \vm ^{\top } \mC \mathbb {E} \rvvu , \shortintertext {applying \cref {assumption:symmetric_standard}} &= \operatorname {tr} \left ( \mC ^{\top } \mC \right ) + \norm {\vm }_2^2 \\ &= \norm {\mC }_\mathrm {F}^2 + \norm {\vm }_2^2 \\ &= \norm {\vlambda }_2^2. \end {align*} Combined with \cref {thm:linearity}, we have \begin {align*} \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda '}\left (\rvvu \right ) }_2^2 = \mathbb {E} \norm { \mathcal {T}_{\vlambda - \vlambda '}\left (\rvvu \right ) }_2^2 = \norm {\vlambda - \vlambda '}_2^2. \end {align*} \par \end{proof}


==> main-pratendproximalsgdbbvi.tex <==


\prAtEndRestatexiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiii}First, we have \begin {align*} \mathbb {E} \norm { \nabla _{\vlambda } f\left (\vlambda ; \rvvu \right ) - \nabla _{\vlambda ^{\prime }} f\left (\vlambda ^{\prime }; \rvvu \right ) }_2^2 &= \mathbb {E} \norm { \nabla _{\vlambda } \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) - \nabla _{\vlambda '} \ell \left (\mathcal {T}_{\vlambda '}\left (\rvvu \right )\right ) }_2^2 \\ &= \mathbb {E} \norm { \frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right )}{\partial \vlambda } g\left (\vlambda , \rvvu \right ) - \frac {\partial \mathcal {T}_{\vlambda '}\left (\rvvu \right )}{\partial \vlambda '} g\left (\vlambda ', \rvvu \right ) }_2^2. \shortintertext {For the linear parameterization, the Jacobian of \(\mathcal {T}_{\vlambda }\) does not depend on \(\vlambda \). Therefore,} &= \mathbb {E} \norm { \frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right )}{\partial \vlambda } \left ( g\left (\vlambda , \rvvu \right ) - g\left (\vlambda ', \rvvu \right ) \right ) }_2^2 \shortintertext {and \cref {thm:jacobian_reparam_inner_original} yields} &= J_{\mathcal {T}}\left (\rvvu \right ) \mathbb {E} \norm { g\left (\vlambda , \rvvu \right ) - g\left (\vlambda ', \rvvu \right ) }_2^2, \end {align*} where \begin {alignat*}{2} J_{\mathcal {T}}\left (\vu \right ) &= 1 + \norm {\vu }_2^2 &&\qquad \text {for the Cholesky family and} \\ J_{\mathcal {T}}\left (\vu \right ) &= 1 + {\lVert \mU ^2 \rVert }_{\mathrm {F}} &&\qquad \text {for the mean-field family.} \end {alignat*} \par From now on, we apply the strategy of~\citet [Theorem 3]{domke_provable_2019} for resolving the randomness \(\rvvu \). That is, \begin {align*} \mathbb {E} J_{\mathcal {T}}\left (\rvvu \right ) \norm { g\left (\vlambda , \rvvu \right ) - g\left (\vlambda ', \rvvu \right ) }_2^2 \nonumber &= J_{\mathcal {T}}\left (\rvvu \right ) \norm { \nabla \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) - \nabla \ell \left (\mathcal {T}_{\vlambda '}\left (\rvvu \right )\right ) }_2^2 \nonumber \shortintertext {from the \(L_{\ell }\)-smoothness of \(f\),} &\leq L_{\ell }^2 \, \mathbb {E} J_{\mathcal {T}}\left (\rvvu \right ) \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2, \nonumber \shortintertext {and applying \cref {thm:u_normsquared_marginalization},} &\leq L_{\ell }^2 \, C\left (d,\varphi \right ) \, \norm { \vlambda - \vlambda ^{\prime } }_2^2 \nonumber \end {align*} \par The last step follows the approach of \citet {kim_practical_2023}, where we convert the quadratic bound into a bound involving the energy. Recall that the \(\mu \)-strongly convexity of \(\ell \) implies \begin {align} \frac {\mu }{2}\norm { \vz ^{\prime } - \vz }_2^2 \leq \ell \left (\vz \right ) - \ell \left (\vz ^{\prime }\right ) - \inner { \nabla \ell \left (\vz ^{\prime }\right ) }{\vz - \vz ^{\prime }}. \end {align} From \cref {thm:difference_t_z_identity}, we have \begin {align*} L_{\ell }^2 \, C\left (d,\varphi \right ) \, \norm { \vlambda - \vlambda ^{\prime } }_2^2 &= L_f^2 \, C\left (d, \varphi \right ) \mathbb {E} \norm { \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right ) }_2^2, \nonumber \shortintertext {and by \(\mu \)-strongly convexity,} &\leq \frac {2 L_{\ell }^2}{\mu } \, C\left (d, \varphi \right ) \mathbb {E} \big ( \ell \left ( \mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) - \ell \left ( \mathcal {T}_{\vlambda '}\left (\rvvu \right )\right ) - \inner { \nabla \ell \left (\mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right )\right ) }{\mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda ^{\prime }}\left (\rvvu \right )} \big ) \nonumber \\ &= \frac {2 L_{\ell }^2}{\mu } \, C\left (d, \varphi \right ) \mathbb {E} \big ( f\left (\vlambda ; \rvvu \right ) - f\left (\vlambda '; \rvvu \right ) - \inner { g\left (\vlambda '; \rvvu \right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda '}\left (\rvvu \right ) } \big ) \nonumber \\ &= \frac {2 L_{\ell }^2}{\mu } \, C\left (d, \varphi \right ) \big ( f\left (\vlambda \right ) - f\left (\vlambda '\right ) - \mathbb {E} \inner { g\left (\vlambda '; \rvvu \right ) }{ \mathcal {T}_{\vlambda }\left (\rvvu \right ) - \mathcal {T}_{\vlambda '}\left (\rvvu \right ) } \big ). \nonumber \shortintertext {Finally, by applying the equality in \cref {thm:innerproduct_z_t},} &= \frac {2 L_{\ell }^2}{\mu } \, C\left (d, \varphi \right ) \big ( f\left (\vlambda \right ) - f\left (\vlambda '\right ) - \inner { \nabla f\left (\vlambda '\right ) }{ \vlambda - \vlambda ' } \big ). \end {align*}\end{proof}

\begin{restatable}[\textbf {Variance Transfer}]{lemma}{prAtEndRestatexiv}\label{thm:prAtEndxiv}\label {thm:variance_transfer} Let \(\ell \) be \(L_{\ell }\)-smooth and \(\mu \)-strongly convex with the variational family satisfying \cref {assumption:variation_family} with the linear parameterization. Also, let \(\widehat {\nabla f}\) be an \(M\)-sample gradient estimator of the energy. Then, { \setlength {\belowdisplayskip }{1.ex} \setlength {\belowdisplayshortskip }{1.ex} \setlength {\abovedisplayskip }{1.ex} \setlength {\abovedisplayshortskip }{1.ex} \[ \mathrm {tr} \, \mathbb {V} \, \widehat {\nabla f}\left (\vlambda \right ) \leq \frac {4 L_{\ell } \kappa \, C\left (d, \varphi \right )}{M} \, \mathrm {B}_{f}\left (\vlambda , \vlambda ^{\prime }\right ) + 2 \, \mathrm {tr} \, \mathbb {V} \, \widehat {\nabla f}\left (\vlambda ^{\prime }\right ), \] }\(\kappa = L_{\ell } / \mu \) is the condition number, \(\mathrm {B}_f\) is the Bregman divergence defined in \cref {thm:es_bregman}, \(C\left (d, \varphi \right ) = d + k_{\varphi }\) for the Cholesky family, and \(C\left (d, \varphi \right ) = 2 k_{\varphi } \sqrt {d} + 1\) for the mean-field family.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxiv}First, the \(M\)-sample gradient estimator is defined as \[ \widehat {\nabla f}\left (\vlambda \right ) = \frac {1}{M} \sum ^{M}_{m=1} \nabla _{\vlambda } f\left (\vlambda ; \rvvu _m\right ), \] where \(\rvvu _m \sim \varphi \). Since \(\rvvu _1, \ldots , \rvvu _m\) are independent and identically distributed, we have \[ \mathrm {tr} \, \mathbb {V} \, \widehat {\nabla f}\left (\vlambda \right ) = \frac {1}{M} \mathrm {tr} \, \mathbb {V} \, \nabla _{\vlambda } f\left (\vlambda ; \rvvu \right ). \] From here, given~\cref {thm:es_bregman}, the proof is identical with that of~\citet [Lemma 8.20]{garrigos_handbook_2023}, except for the constants.\end{proof}

\begin{restatable}[]{theorem}{prAtEndRestatexv}\label{thm:prAtEndxv}\label {thm:strongly_convex_proximal_sgd} Let \(\ell \) be \(L_{\ell }\)-smooth and \(\mu \)-strongly convex. Then, BBVI with proximal SGD in \cref {eq:proxsgd}, \(M\)-Monte Carlo samples, a variational family satisfying \cref {assumption:variation_family}, the linear parameterization, and a fixed stepsize \(0 < \gamma \leq \frac {M}{2 L_{\ell } \, \kappa \, C\left (d, \varphi \right ) }\), the iterates satisfy \[ \mathbb {E}\norm { \vlambda _T - \vlambda ^* }_2^2 \leq {\left (1 - \gamma \mu \right )}^{T} {\lVert \vlambda _0 - \vlambda ^2 \rVert }_2^2 + \frac {2 \gamma \sigma ^2}{\mu }, \] where \(\kappa = L_{\ell } / \mu \) is the condition number, \(\sigma ^2\) is defined in \cref {thm:optimum_gradient_variance}, \(\vlambda ^* = \argmin _{\vlambda \in \Lambda } F\left (\vlambda \right )\), \(C(d, \varphi ) = d + k_{\varphi }\) for the Cholesky family, and \(C(d, \varphi ) = 2 k_{\varphi } \sqrt {d} + 1 \) for the mean-field family.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxv}Provided that \begin {enumerate}[label=\textbf {(A.\labelcref *{thm:strongly_convex_proximal_sgd}.\arabic *)},itemsep=-1ex] \item the energy \(f\) is \(\mu \)-strongly convex,~\label {eq:proximal_strongly_log_concave_cond1} \item the energy \(f\) is \(L_{\ell }\)-smooth,~\label {eq:proximal_strongly_log_concave_cond7} \item the regularizer \(h\) is convex,~\label {eq:proximal_strongly_log_concave_cond2} \item the regularizer \(h\) is lower semi-continuous,~\label {eq:proximal_strongly_log_concave_cond3} \item the convex expected smoothness condition holds,~\label {eq:proximal_strongly_log_concave_cond5} \item the variance transfer condition holds, and~\label {eq:proximal_strongly_log_concave_cond8} \item the gradient variance \(\sigma ^2\) at the optimum is finite such that \(\sigma ^2 < \infty \),~\label {eq:proximal_strongly_log_concave_cond6} \end {enumerate} the proof is identical to that of \citet [Theorem 11.9]{garrigos_handbook_2023}, which is based on the results of~\citet [Corollary A.2]{gorbunov_unified_2020}. \par In our setting, \begin {enumerate}[itemsep=-1ex] \item [\labelcref *{eq:proximal_strongly_log_concave_cond1}] is established by~\cref {thm:energy_convex}, \item [\labelcref *{eq:proximal_strongly_log_concave_cond7}] is established by~\cref {thm:energy_smooth}, \item [\labelcref *{eq:proximal_strongly_log_concave_cond2}] is trivially satisfied since \(h\) is the negative entropy, \item [\labelcref *{eq:proximal_strongly_log_concave_cond3}] is trivially satisfied since \(h\) is continuous, \item [\labelcref *{eq:proximal_strongly_log_concave_cond5}] is established in \cref {thm:es_bregman}, \item [\labelcref *{eq:proximal_strongly_log_concave_cond8}] is established in \cref {thm:variance_transfer}, \item [\labelcref *{eq:proximal_strongly_log_concave_cond6}] is established in \cref {thm:optimum_gradient_variance}. \end {enumerate} \par The only difference is that, we replace the constant \(L_{\mathrm {max}}\) in the proof of \citeauthor {garrigos_handbook_2023} to \({L_{\ell } \kappa \, C\left (d, \varphi \right )}/{M}\). This stems from the different constants in the variance transfer condition.\end{proof}

\begin{restatable}[]{theorem}{prAtEndRestatexvi}\label{thm:prAtEndxvi}\label {thm:complexity_strongly_convex_proximal_sgd} Let \(\ell \) be \(L_{\ell }\)-smooth and \(\mu \)-strongly convex. Then, for any \(\epsilon > 0\), BBVI with proximal SGD in \cref {eq:proxsgd}, \(M\)-Monte Carlo samples, a variational family satisfying \cref {assumption:variation_family}, and the linear parameterization guarantees \(\mathbb {E} \norm {\vlambda _T - \vlambda ^*}_2^2 \leq \epsilon \) if {\setlength {\belowdisplayskip }{1.0ex} \setlength {\belowdisplayshortskip }{1.ex} \setlength {\abovedisplayskip }{.5ex} \setlength {\abovedisplayshortskip }{.5ex} \[ \gamma = \min \left (\frac {\epsilon }{2} \frac {\mu }{2 \sigma ^2}, \frac {M}{2 L_{\ell } \, \kappa \, C\left (d, \varphi \right )} \right ), \qquad T \geq \max \left ( \frac {1}{\epsilon } \frac {4 \sigma ^2}{\mu ^2}, \frac {2 \kappa ^2 \, C\left (d, \varphi \right )}{M} \right ) \log \left ( \frac {2 \norm {\vlambda _0 - \vlambda ^*}}{\epsilon } \right ), \] }where \(\kappa = L_{\ell } / \mu \), \(\sigma ^2\) is defined in \cref {thm:optimum_gradient_variance}, \(\vlambda ^* = \argmin _{\vlambda \in \Lambda } F\left (\vlambda \right )\), \(C(d, \varphi ) = d + k_{\varphi }\) for the Cholesky family, and \(C(d, \varphi ) = 2 k_{\varphi } \sqrt {d} + 1 \) for the mean-field family.\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvi}\vspace {-2ex} This is a corollary of the fixed stepsize convergence guarantee in \cref {thm:strongly_convex_proximal_sgd} as shown by~\citet [Corollary 11.10]{garrigos_handbook_2023}. They guarantee an \(\epsilon \)-accurate solution as long as \[ \gamma = \min \left ( \frac {\epsilon }{2} \frac {2}{2 \sigma ^*_{\mathrm {F}}}, \frac {1}{2 L_{\mathrm {max}}} \right ),\quad T \geq \max \left ( \frac {1}{\epsilon } \frac {4 \sigma _{\mathrm {F}}^*}{\mu ^2}, \frac {2 L_{\mathrm {max}}}{\mu }\right ) \log \left ( \frac {2 \norm {\vlambda _0 - \vlambda ^*}}{\epsilon } \right ). \] In our notation, \(\sigma ^*_{\mathrm {F}} = \sigma ^2\) and \(L_{\mathrm {max}} = {L_{\ell } \kappa C\left (d, \varphi \right )}/{M}\).\end{proof}

\begin{restatable}[]{theorem}{prAtEndRestatexvii}\label{thm:prAtEndxvii}\label {thm:strongly_convex_proximal_sgd_decgamma} Let \(\ell \) be \(L_{\ell }\)-smooth and \(\mu \)-strongly convex. Then, BBVI with proximal SGD in \cref {eq:proxsgd}, the \(M\)-sample reparameterization gradient estimator, a variational family satisfying \cref {assumption:variation_family}, the linear parameterization, \(T \geq 4 T_{\kappa } \), and a stepsize schedule of \[ \gamma _t = \begin {cases} \frac {M}{ 2 L_{\ell } \kappa C\left (d, \varphi \right ) } & \quad \text {for}\quad t \leq 4 T_{\kappa } \\ \frac {2t + 1}{ {\left (t+1\right )}^2 \mu } & \quad \text {for}\quad t > 4 T_{\kappa }, \\ \end {cases} \] where \(T_{\kappa } = {\lceil \kappa ^2 C\left (d, \varphi \right ) M^{-1} \rceil }\), \(\kappa = L_{\ell } / \mu \) is the condition number, \(C(d, \varphi ) = d + k_{\varphi }\) for the Cholesky family, and \(C(d, \varphi ) = 2 k_{\varphi } \sqrt {d} + 1 \) for the mean-field family, then the iterates satisfy \[ \mathbb {E}\norm { \vlambda _T - \vlambda ^* }_2^2 \leq \frac { 16 \, T_{\kappa }^2 \, \norm {\vlambda _0 - \vlambda ^*}_2^2 }{ \mathrm {e}^2 T^2} + \frac {8 \sigma ^2}{\mu ^2 T} \] where \(\sigma ^2\) is defined in \cref {thm:optimum_gradient_variance}, \(\mathrm {e}\) is Euler's constant, and \(\vlambda ^* = \argmin _{\vlambda \in \Lambda } F\left (\vlambda \right )\).\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxvii}\vspace {-1ex} Under our assumptions, \cref {thm:strongly_convex_proximal_sgd} holds, of which the proof is essentially obtaining the recursion \begin {align*} \mathbb {E} \norm {\vlambda _{t+1} - \vlambda ^*}_2^2 = \left (1 - \gamma _t \mu \right ) \mathbb {E} \norm {\vlambda _{t} - \vlambda ^*}_2^2 + 2 \gamma ^2_t \sigma ^2. \end {align*} Instead of a fixed stepsize, we can apply the decreasing stepsize rule in the proof statement, then which the proof becomes identical to that of~\citet [Theorem 3.2]{gower_sgd_2019}. We only need to replace \(\mathcal {L}\) with \(L_{\mathrm {max}}\) in the proof of \citet [Theorem 11.9]{garrigos_handbook_2023}. This, in our notation, is \(L_{\mathrm {max}} = {L_{\ell } \kappa C\left (d, \varphi \right )}/{M}\).\end{proof}

\prAtEndRestatexviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxviii}The computational complexity follows from the smallest number of iterations \(T\) such that \[ \mathbb {E}\norm { \vlambda _T - \vlambda ^* }_2^2 \leq \frac { 16 T_{\kappa }^2 \norm {\vlambda _0 - \vlambda ^*}_2^2 }{ \mathrm {e}^2 T^2} + \frac {8 \sigma ^2}{\mu ^2 T} \leq \epsilon \] \par By multiplying both sides with \(T^2\) as \begin {alignat}{3} T^2 \epsilon - \frac {8 \sigma ^2}{\mu ^2} T - \frac { 16 T_{\kappa }^2 \norm {\vlambda _0 - \vlambda ^*}_2^2 }{ \mathrm {e}^2} \geq 0, \end {alignat} we can see that we are looking for the smallest positive integer that is larger than the solution of a quadratic equation with respect to \(T\). This is given as \[ T \geq \frac { \frac {8 \sigma ^2}{\mu ^2} + \sqrt { {\left (\frac {8 \sigma ^2}{\mu ^2}\right )}^2 + 64 \epsilon \frac {T_{\kappa }^2 \, \norm {\vlambda _0 - \vlambda ^*}_2^2 }{ \mathrm {e}^2} } }{2 \epsilon }. \] Applying the inequality \(\sqrt {a + b} \leq \sqrt {a} + \sqrt {b}\), \begin {align*} \frac { \frac {8 \sigma ^2}{\mu ^2} + \sqrt { {\left (\frac {8 \sigma ^2}{\mu ^2}\right )}^2 + 64 \epsilon \frac {T_{\kappa }^2 \, \norm {\vlambda _0 - \vlambda ^*}_2^2 }{ \mathrm {e}^2} } }{2 \epsilon } &\leq \frac { \frac {8 \sigma ^2}{\mu ^2} + {\left (\frac {8 \sigma ^2}{\mu ^2}\right )} + \sqrt {64 \epsilon \frac {T_{\kappa }^2 \, \norm {\vlambda _0 - \vlambda ^*}_2^2 }{ \mathrm {e}^2} } }{2 \epsilon } \\ &= \frac { \frac {16 \sigma ^2}{\mu ^2} + \sqrt {\epsilon } \, \frac { 8 T_{\kappa } \, {\lVert \vlambda _0 - \vlambda ^* \rVert }_2 }{ \mathrm {e}} } {2 \epsilon } \\ &= \frac {8 \sigma ^2}{\mu ^2 \, \epsilon } + \frac { 4 T_{\kappa } \norm {\vlambda _0 - \vlambda ^*}_2 }{\mathrm {e} \, \sqrt {\epsilon }}. \end {align*} \par Thus, \(\mathbb {E} \norm {\vlambda _T - \vlambda ^*}_2^2 \leq \epsilon \) can be satisfied with a number of iterations at least \begin {align*} T &\geq \max \left ( \frac {8 \sigma ^2}{\mu ^2 \, \epsilon } + \frac { 4 T_{\kappa } \norm {\vlambda _0 - \vlambda ^*}_2 }{\mathrm {e} \, \sqrt {\epsilon }},\;\; 4 T_{\kappa } \right ). \end {align*}\end{proof}


==> main-pratendregularity.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndii}The entropic regularizer is \[ h\left (\vlambda \right ) = -\mathrm {H}\left (\varphi \right ) - \sum ^{d}_{i=1} \log \phi \left (s_{i}\right ), \] and depends only on the diagonal elements \(s_{1}, \ldots , s_{d}\) of \(\mC \). The Hessian of \(h\) is then a diagonal matrix, where only the entries that correspond to \(s_{1}, \ldots , s_{d}\) are non-zero. The Lipschitz smoothness constant is then the constant \(L_h < \infty \) that satisfies \[ \frac {\partial ^2 h\left (\vlambda \right )}{\partial s_{i}^2} = -\frac {\mathrm {d}^2 \log \phi }{ \mathrm {d} s_{i}^2} < L_h \] for all \(i = 1, \ldots , d\), which is the smoothness constant of \(s_{i} \mapsto \log \phi \left (s_{i}\right )\).\end{proof}


==> main-pratendsgdbbvi.tex <==


\begin{restatable}[]{theorem}{prAtEndRestatexi}\label{thm:prAtEndxi}\label {thm:nonconvex_sgd_convergence} Let the variational family satisfy \cref {assumption:variation_family}, the likelihood satisfy~\cref {assumption:quadratic_growth}, and the assumptions of \cref {thm:elbo_smooth} hold such that the ELBO, \(F\), is \(L_F\)-smooth with \(L_F = L_{\ell } + L_{\phi } + L_{s}\). Then, if the stepsize satisfy \(\gamma < {1}/{L_F}\), the iterates of BBVI with SGD and the \(M\)-sample reparameterization gradient estimator satisfy {\setlength {\belowdisplayskip }{.0ex} \setlength {\belowdisplayshortskip }{.0ex} \setlength {\abovedisplayskip }{1.0ex} \setlength {\abovedisplayshortskip }{1.0ex} \begin {align*} \min _{0 \leq t \leq T-1} \mathbb {E} \norm {\nabla F\left (\vlambda _t\right ) }_2^2 &\leq \gamma \frac {2 L_F L_{\ell } \kappa \, C\left (d, \varphi \right ) }{M} \, \left ( \lVert { \bar {\vz }_{\mathrm {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + 2 \left (F^* - f^*_{\mathrm {L}}\right ) \right ) \\ &\quad + \frac {2}{\gamma T} {\left (1 + \gamma ^2 \frac {4 L_{F} L_{\ell } \, \kappa }{ M} \, C\left (d, \varphi \right ) \right )}^T \left ( F\left (\vlambda _0\right ) - F^* \right ). \end {align*} }where \begin {alignat*}{2} \bar {\vz }_{\mathrm {joint}} &= \mathrm {proj}_{\ell }\left (\vz \right ) &&\quad \text {is the projection of \(\vz \) onto set of minimizers of \(\ell \)} \\ \bar {\vz }_{\mathrm {like}} &= \mathrm {proj}_{\ell _{\mathrm {like}}}\left (\vz \right ) &&\quad \text {is the projection of \(\vz \) onto set of minimizers of \(\ell _{\mathrm {like}}\),} \\ \kappa &= \nicefrac {L_{\ell }}{\mu } &&\quad \text {is the condition number,} \\ F^* &= \inf _{\vlambda \in \Lambda } F\left (\vlambda \right ), \\ {\ell }^*_{\mathrm {like}} &= \inf _{\vlambda \in \mathbb {R}^d} {\ell }_{\mathrm {like}}\left (\vz \right ), \\ C(d, \varphi ) &= d + k_{\varphi } && \quad \text {for the Cholesky nonlinear,} \\ C(d, \varphi ) &= 2 k_{\varphi } \sqrt {d} + 1 && \quad \text {for the mean-field nonlinear,} \\ M & && \quad \text {is the number of Monte Carlo samples.} \end {alignat*}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxi}\citet [Theorem 2]{khaled_better_2023} show that, if the objective function \(F\) is \(L_F\)-smooth and the stochastic gradients satisfy the \(ABC\) given as \[ \mathbb {E} \lVert { \widehat {\nabla F}\left (\vlambda \right ) \rVert }_2^2 \leq A \left (F\left (\vlambda \right ) - F^*\right ) + B \norm {\nabla F}_2^2 + C \] for some \(0 < A, B, C < \infty \), SGD guarantees \[ \min _{0 \leq t \leq T-1} \mathbb {E} \norm {\nabla F\left (\vlambda _t\right ) }_2^2 \leq L_{F} C \gamma + \frac {2 {\left (1 + L_{F} \gamma ^2 A\right )}^T }{ \gamma T } \left ( F\left (\vlambda _0\right ) - F^* \right ). \] \par Under the conditions of \cref {thm:elbo_smooth}, \(F\) is \(L_F\)-smooth with \(L_F = L_{\ell } + L_s + L_{\phi }\). Furthermore, under \cref {assumption:quadratic_growth},~\cite {kim_practical_2023} show that the Monte Carlo gradient estimates satisfy \begin {align*} \mathbb {E} \lVert { \widehat {\nabla F}\left (\vlambda \right ) \rVert }_2^2 &\leq \frac { 4 L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} \left (F\left (\vlambda \right ) - F^*\right ) + B \norm {\nabla F}_2^2 \\ &\quad + \frac { 2 L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} {\lVert \bar {\vz }_{\mathrm {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + \frac { 4 L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} \left (F^* - \ell _{\mathrm {like}}^*\right ), \end {align*} \par This means that the \(ABC\) condition is satisfied with constants \[ A = \frac {4 L_{\ell }^2}{\mu M} C\left (d, \varphi \right ), \qquad B = 1, \qquad C = \frac {2 L_{\ell }^2}{\mu M} C\left (d, \varphi \right ) \lVert { \bar {\vz }_{\mathrm {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + \frac {4 L_{\ell }^2}{\mu M} C\left (d, \varphi \right ) \left (F^* - {\ell }^*_{\mathrm {like}}\right ). \] \par Plugging these constants in, we obtain \begin {align*} \min _{0 \leq t \leq T-1} \mathbb {E} \norm {\nabla f\left (\vlambda _t\right ) }_2^2 &\leq \gamma \frac {2 L_F L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} \left ( \lVert { \bar {\vz }_{\text {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + 2 \left (F^* - \ell ^*_{\mathrm {like}}\right ) \right ) \\ &\quad + \frac {2}{\gamma T} {\left (1 + \gamma ^2 L_{F} \frac {4 L_{\ell }^2}{\mu M} C\left (d, \varphi \right ) \right )}^T \left ( F\left (\vlambda _0\right ) - F^* \right ). \end {align*} Substituting the condition number yields the stated result.\end{proof}

\prAtEndRestatexii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndxii}As a corollary to \cref {thm:nonconvex_sgd_convergence}, \citet [Corollary 1]{khaled_better_2023} show that, for an \(L_F\)-smooth objective function \(F\), a gradient estimator satisfying the \textit {ABC} condition, an \(\epsilon \)-stationary point can be encountered if \[ \gamma = {\min \left (\frac {1}{\sqrt {L_F A T}}, \frac {1}{L_F B}, \frac {\epsilon }{2 L_F C} \right ),\qquad } T \geq \frac {12 \left ( F\left (\vlambda _0\right ) - F^* \right ) L_F}{\epsilon ^2} \max \left ( B, \frac {12 \left ( F\left (\vlambda _0\right ) - F^* \right ) A}{\epsilon ^2}, \frac {2 C}{\epsilon ^2} \right ). \] \par Under \cref {assumption:quadratic_growth},~\cite {kim_practical_2023} show that the Monte Carlo gradient estimates satisfy \begin {align*} \mathbb {E} \lVert { \widehat {\nabla F}\left (\vlambda \right ) \rVert }_2^2 &\leq \frac { 4 L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} \left (F\left (\vlambda \right ) - F^*\right ) + B \norm {\nabla F}_2^2 \\ &\quad + \frac { 2 L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} {\lVert \bar {\vz }_{\mathrm {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + \frac { 4 L_{\ell }^2 C\left (d, \varphi \right ) }{\mu M} \left (F^* - \ell _{\mathrm {like}}^*\right ), \end {align*} This means that the \(ABC\) condition is satisfied with constants \[ A = \frac {4 L_f^2}{\mu M} C\left (d, \varphi \right ), \qquad B = 1, \qquad C = \frac {2 L_f^2}{\mu M} C\left (d, \varphi \right ) \left ( \lVert { \bar {\vz }_{\mathrm {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + 2 \left (F^* - f^*_{\mathrm {L}}\right ) \right ). \] where \begin {alignat*}{2} \bar {\vz }_{\mathrm {joint}} &= \mathrm {proj}_{\ell }\left (\vz \right ) &&\quad \text {is the projection of \(\vz \) onto set of minimizers of \(\ell \)} \\ \bar {\vz }_{\mathrm {like}} &= \mathrm {proj}_{\ell _{\mathrm {like}}}\left (\vz \right ) &&\quad \text {is the projection of \(\vz \) onto set of minimizers of \(\ell _{\mathrm {like}}\),} \\ F^* &= \inf _{\vlambda \in \Lambda } F\left (\vlambda \right ), \\ \ell ^*_{\mathrm {like}} &= \inf _{\vlambda \in \mathbb {R}^d} \ell _{\mathrm {like}}\left (\vz \right ), \\ C(d, \varphi ) &= d + k_{\varphi } && \quad \text {for the Cholesky family,} \\ C(d, \varphi ) &= 2 k_{\varphi } \sqrt {d} + 1 && \quad \text {for the mean-field family,} \\ M & && \quad \text {is the number of Monte Carlo samples.} \end {alignat*} \par Plugging these constants in, we obtain \begin {align*} T &\geq \frac {12 \left ( F\left (\vlambda _0\right ) - F^* \right ) L_F}{\epsilon ^2} \max \left (1, \frac {48 \left ( F\left (\vlambda _0\right ) - F^* \right ) L_{\ell }^2 C\left (d, \varphi \right )}{\mu M \epsilon ^2}, \frac {8 L_{\ell }^2 C\left (d, \varphi \right ) \left ( {\lVert \bar {\vz }_{\mathrm {joint}} - \bar {\vz }_{\mathrm {like}} \rVert }_2^2 + \left (F^* - \ell ^*_{\mathrm {like}}\right ) \right ) }{ \mu M \epsilon ^2} \right ) \\ &= \mathcal {O}\left ( \frac { {\left ( F\left (\vlambda _0\right ) - F^* \right )}^2 L_F L_{\ell }^2 C\left (d\right )}{\mu M \epsilon ^4} \right ), \end {align*} where we omitted the dependence on \(k_{\varphi }\) and the minimizers of \(\ell \) and \(\ell _{\mathrm {like}}\).\end{proof}


==> main-pratendsmoothness.tex <==


\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndv}For notational clarity, we will occasionally represent \(\mathcal {T}_{\vlambda }\) as \[ \mathcal {T}_{\vlambda }\left (\rvvu \right ) = \mathcal {T}\left (\vlambda ; \rvvu \right ), \] such that \(\mathcal {T}_i\left (\vlambda ; \rvvu \right )\) denotes the \(i\)th component of \(\mathcal {T}_{\vlambda }\). \par \par By the Leibniz and chain rule, the Hessian of the energy \(f\) follows as \begin {align*} \nabla ^2 f\left (\vlambda \right ) &= \mathbb {E} \nabla ^2_{\vlambda } \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) \\ &= \underbrace { \mathbb {E} {\left (\frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda }\right )}^{\top } \nabla ^2 \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) \frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda } }_{\triangleq T_{\text {lin}}} \;+\; \underbrace { \mathbb {E} \sum ^{d}_{i=1} \mathrm {D}_i \ell \left ( \mathcal {T}_{\vlambda }\left (\rvvu \right ) \right ) \frac { \partial ^2 \mathcal {T}_{i}\left (\vlambda ; \rvvu \right ) }{ \partial \vlambda ^2 } }_{\triangleq T_{\text {non}}}. \end {align*} When \(\mathcal {T}\) is linear with respect to \(\vlambda \), it is clear that we have \begin {equation} \frac { \partial ^2 \mathcal {T}_{i}\left (\vlambda ; \rvvu \right ) }{ \partial \vlambda ^2 } = \boldupright {0}. \label {thm:energy_smooth_second_derivative} \end {equation} Then, \(T_{\text {non}}\) is zero. In contrast, \(T_{\text {lin}}\) appears for both the linear and nonlinear cases. Therefore, \(T_{\text {non}}\) fully characterizes the effect of nonlinearity in the reparameterization function. \par Now, the triangle inequality yields \begin {align*} {\lVert \nabla ^2 f\left (\vlambda \right ) \rVert }_2 = \norm {T_{\text {lin}} + T_{\text {non}}}_2 \leq \norm {T_{\text {lin}}}_2 + \norm {T_{\text {non}}}_2, \end {align*} where equality is achieved when either term is 0. On the contrary, the reverse triangle inequality states that \begin {align*} \abs { \norm {T_{\text {lin}}}_2 - \norm {T_{\text {non}}}_2 } \leq {\lVert \nabla ^2 f\left (\vlambda \right ) \rVert }_2. \end {align*} This implies that, if either \(T_{\text {lin}}\) or \(T_{\text {non}}\) is unbounded, the Hessian is not bounded. Thus, ensuring that \(T_{\text {lin}}\) and \(T_{\text {non}}\) are bounded is sufficient and necessary to establish that \(f\) is smooth. \par \paragraph {Proof of \labelcref *{item:linear_phi_energy_smooth}} The bound on the linear part, \(T_{\text {lin}}\), follows from \cref {thm:orthogonal_decomp_expectation} as \begin {align*} \norm {T_{\text {lin}}}_2 &= \norm { \mathbb {E} {\left (\frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda }\right )}^{\top } \nabla ^2 \ell \left (\mathcal {T}_{\vlambda }\left (\rvvu \right )\right ) \frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda } }_2 \\ &\leq L_{\ell } \norm { \mathbb {E} {\left (\frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda }\right )}^{\top } \frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda } }_2, \shortintertext {and from the 1-Lipschitzness of \(\phi \), \cref {thm:reparam_jacobian_bounded} yields} &\leq L_{\ell }. \end {align*} \par When \(\phi \) is linear, it immediately follows from \cref {thm:energy_smooth_second_derivative} that \[ {\lVert \nabla ^2 f\left (\vlambda \right ) \rVert }_2 = \norm { T_{\text {lin}} }_2 \leq L_{\ell }, \] which is tight as shown by \citet [Theorem 6]{domke_provable_2020}. \par \paragraph {Proof of \labelcref *{item:nonlinear_phi_energy_smooth}} For the nonlinear part \(T_{\text {non}}\), we use the fact that \({\mathcal {T}}_{i}\left (\vlambda ; \rvvu \right )\) is given as \[ {\mathcal {T}}_{i}\left (\vlambda ; \rvvu \right ) = m_i + \phi \left (s_i\right ) \rvu _i +\sum _{j \neq i} L_{ij} \rvu _j. \] The second derivative of \(\mathcal {T}_{i}\) is clearly non-zero only for the nonlinear part involving \(s_1, \ldots , s_d\). Thus, \(T_{\text {non}}\) follows as \begin {align*} T_{\text {non}} &= \mathbb {E} \sum ^{d}_{i=1} \mathrm {D}_i \ell \left ( \mathcal {T}_{\vlambda }\left (\rvvu \right ) \right ) \frac { \partial ^2 {\mathcal {T}}_{i}\left (\vlambda ; \rvvu \right ) }{ \partial \vlambda ^2 } \\ &= \mathbb {E} \sum ^{d}_{i=1} g_i\left (\vlambda ; \rvvu \right ) \frac { \partial ^2 {\mathcal {T}}_{i}\left (\vlambda ; \rvvu \right ) }{ \partial \vlambda ^2 } \\ &= \begin {bmatrix} \cdot & \cdot & \cdot \\ \cdot & \mathbb {E} \sum ^{d}_{i=1} g_{i}\left (\vlambda ; \rvvu \right ) \frac { \partial ^2 \mathcal {T}_{i}\left (\vlambda ; \rvvu \right ) }{ \partial \vs ^2 } & \cdot \\ \cdot & \cdot & \cdot \end {bmatrix}. \end {align*} Furthermore, the second-order derivatives with respect to \(s_1, \ldots , s_d\) are given as \[ \frac { \partial ^2 \mathcal {T}_i\left (\vlambda ; \rvvu \right ) }{ \partial s_j^2 } = \mathbb {1}_{i = j} \phi ''\left (s_j\right ). \] Considering this, the only non-zero block of \(T_{\mathrm {non}}\) forms a diagonal matrix as \begin {align*} \mathbb {E} \sum ^{d}_{i=1} g_{i}\left (\vlambda ; \rvvu \right ) \frac { \partial ^2 {\mathcal {T}}_{i}\left (\vlambda ; \rvvu \right ) }{ \partial \vs } &= \begin {bmatrix} \mathbb {E} g_1\left (\vlambda ; \rvvu \right ) \frac { \partial ^2 {\mathcal {T}}_{1}\left (\vlambda ; \rvvu \right ) }{ \partial s_1^2 } & & \\ & \ddots & \\ & & \mathbb {E} g_d\left (\vlambda ; \rvvu \right ) \frac { \partial ^2 {\mathcal {T}}_{d}\left (\vlambda ; \rvvu \right ) }{ \partial s_d^2 } \end {bmatrix} \\ &= \begin {bmatrix} \mathbb {E} g_1\left (\vlambda ; \rvvu \right ) \, \phi ^{\prime \prime }\left (s_1\right ) \rvu _1 & & \\ & \ddots & \\ & & \mathbb {E} g_d\left (\vlambda ; \rvvu \right ) \, \phi ^{\prime \prime }\left (s_d\right ) \rvu _d \end {bmatrix} \end {align*} This implies that the only non-zero entries of \(T_{\mathrm {non}}\) lie on its diagonal. Since the \(\ell _2\) norm of a diagonal matrix is the value of the maximal diagonal element, \[ \norm {T_{\mathrm {non}}}_2 \leq \max _{i=1, \ldots , d} \mathbb {E} g_i\left (\vlambda ; \rvvu \right ) \, \phi ^{\prime \prime }\left (s_i\right ) \rvu _i \leq L_s, \] where \(L_s\) is finite constant if \cref {assumption:peculiar_smoothness} holds. On the contrary, if a finite \(L_s\) does not exist, \(\norm {T_{\mathrm {non}}}_2\) cannot be bounded. Therefore, the energy is smooth if and only if \cref {assumption:peculiar_smoothness} holds. When it does, the energy \(f\) is \(L_f + L_s\) smooth.\end{proof}


==> main-pratendsmoothnessboundedjacobian.tex <==


\begin{restatable}[]{lemma}{prAtEndRestateiv}\label{thm:prAtEndiv}\label {thm:reparam_jacobian_bounded} For a \(1\)-Lipschitz diagonal conditioner \(\phi \), the Jacobian of the location-scale reparameterization function \(\mathcal {T}_{\vlambda }\) satisfies \[ \norm { \mathbb {E} \, {\left ( \frac { \partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{ \partial \vlambda } \right )}^{\top } \frac { \partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{ \partial \vlambda } }_2 \leq 1. \]\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiv}For notational clarity, we will occasionally represent \(\mathcal {T}_{\vlambda }\) as \[ \mathcal {T}_{\vlambda }\left (\rvvu \right ) = \mathcal {T}\left (\vlambda ; \rvvu \right ), \] such that \(\mathcal {T}_i\left (\vlambda ; \rvvu \right )\) denotes the \(i\)th component of \(\mathcal {T}_{\vlambda }\). \par From the definition of \(\mathcal {T}_{\vlambda }\), it is straightforward to notice that its Jacobian is the concatenation of 3 block matrices \[ \mJ _{\vm } = \frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right )}{ \partial \vm }, \qquad \mJ _{\vs } = \frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right )}{ \partial \vs },\; \text {and} \quad \mJ _{\mL } = \frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right )}{ \partial \mathrm {vec}\left (\mL \right )}. \] \par The \(\vm \) block form a deterministic identity matrix \[ \mJ _{\vm } = \frac {\partial \mathcal {T}_{\vlambda }\left (\vu \right )}{ \partial \vm } = \boldupright {I}, \] which is shown by \citep [Lemma 4]{domke_provable_2020}. \par The proof strategy is as follows: we will directly compute the squared Jacobian through block matrix multiplication. The key is that, after expectation, the resulting matrix becomes diagonal. Then, the \(\ell _2\) operator norm, or maximal eigenvalue, follows trivially as the maximal diagonal element. \par First, \begin {align*} \mathbb {E} \, {\left (\frac {\partial \mathcal {T}\left (\vlambda ; \rvvu \right ) }{\partial \vlambda }\right )}^{\top } \frac {\partial \mathcal {T}\left (\vlambda ;\rvvu \right ) }{\partial \vlambda } &= \mathbb {E} {\begin {bmatrix} \mJ _{\vm }^{\top } \\ \rvmJ _{\vs }^{\top } \\ \rvmJ _{\mL }^{\top } \end {bmatrix}} \begin {bmatrix} \mJ _{\vm } & \rvmJ _{\vs } & \rvmJ _{\mL } \end {bmatrix} \\ &= \mathbb {E} \begin {bmatrix} \mJ _{\vm }^{\top } \mJ _{\vm } & \mJ _{\vm }^{\top } \rvmJ _{\vs } & \mJ _{\vm }^{\top } \rvmJ _{\mL } \\ \rvmJ _{\vs }^{\top } \mJ _{\vm } & \rvmJ _{\vs }^{\top } \rvmJ _{\vs } & \rvmJ _{\vs }^{\top } \rvmJ _{\mL } \\ \rvmJ _{\mL }^{\top } \rvmJ _{\vm } & \rvmJ _{\mL }^{\top } \rvmJ _{\vs } & \rvmJ _{\mL }^{\top } \rvmJ _{\mL } \end {bmatrix} \\ &= \begin {bmatrix} \boldupright {I} & \mathbb {E} \rvmJ _{\vs } & \mathbb {E} \rvmJ _{\mL } \\ \mathbb {E} \rvmJ _{\vs }^{\top } & \mathbb {E} \rvmJ _{\vs }^{\top } \rvmJ _{\vs } & \mathbb {E} \rvmJ _{\vs }^{\top } \rvmJ _{\mL } \\ \mathbb {E} \rvmJ _{\mL }^{\top } & \mathbb {E} \rvmJ _{\mL }^{\top } \rvmJ _{\vs } & \mathbb {E} \rvmJ _{\mL }^{\top } \rvmJ _{\mL } \end {bmatrix}. \end {align*} \par For \(\rvmJ _{\vs }\), the entries are \[ \frac { \partial {\mathcal {T}}_i\left (\rvvu \right ) }{ \partial s_j } = \phi ^{\prime }\left (s_i\right ) \rvu _j \mathbb {1}_{i = j}, \] which is a diagonal matrix. Thus, by~\cref {assumption:symmetric_standard}, \[ \mathbb {E}\rvmJ _{\vs } = \boldupright {O},\qquad \mathbb {E} \rvmJ _{\vs }^{\top } \rvmJ _{\vs } = {\mathrm {diag}\left ({\vphi ^{\prime }\left (\vs \right )}\right )}^2. \] \par For \(\mJ _{\vs }\), the entries are \[ \frac { \partial {\mathcal {T}}_i\left (\vlambda ; \rvvu \right ) }{ \partial L_{jk} } = u_{k} \mathbb {1}_{i = j}. \] To gather some intuition, the case of \(d=4\) looks like the following: \[ \rvmJ _{\mL } = {\setcounter {MaxMatrixCols}{20} \begin {bmatrix} \rvu _2 & \rvu _3 & \rvu _4 & & & & & & & & & \\ & & & \rvu _1 & \rvu _3 & \rvu _4 & & & & & & \\ & & & & & & \rvu _1 & \rvu _2 & \rvu _4 & & & \\ & & & & & & & & & \rvu _1 & \rvu _2 & \rvu _3 \end {bmatrix}. } \] It is crucial to notice that the \(i\)th row does \textit {not} include \(\rvu _i\). This means that, the matrix \(\rvmJ _{\vs }^{\top } \rvmJ _{\mL }\) has entries that are either 0, or \(\phi ^{\prime }\left (s_i\right ) \rvu _i \rvu _j \) for \(i \neq j\), which is \( \mathbb {E} \phi ^{\prime }\left (s_i\right ) \rvu _i \rvu _j = 0\) by \cref {assumption:symmetric_standard}. Therefore, \[ \mathbb {E} \rvmJ _{\vs }^{\top } \rvmJ _{\mL } = \boldupright {O}. \] Finally, the elements of \(\rvmJ _{\mL }^{\top } \rvmJ _{\mL }\) are \[ \mathbb {E} \sum ^d_{i=0} \frac { \partial {\mathcal {T}}_i\left (\vlambda ; \rvvu \right ) }{ \partial L_{jk} } \frac { \partial {\mathcal {T}}_i\left (\vlambda ; \rvvu \right ) }{ \partial L_{lm} } = \mathbb {E} \sum ^d_{i=0} \rvu _{k} \rvu _{m} \mathbb {1}_{i = j} \, \mathbb {1}_{i = l} = \mathbb {1}_{j = l} \left ( \mathbb {E} \rvu _{k} \rvu _{m} \right ) = \mathbb {1}_{j = l} \mathbb {1}_{k = m}, \] where the last equality follows from~\cref {assumption:symmetric_standard}, which forms an identity matrix as \[ \mathbb {E}\rvmJ _{\mL }^{\top } \rvmJ _{\mL } = \boldupright {I}. \] \par Therefore, the expected-squared Jacobian is now \begin {align*} \mathbb {E} \, {\left (\frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda }\right )}^{\top } \frac {\partial \mathcal {T}_{\vlambda }\left (\rvvu \right ) }{\partial \vlambda } &= \begin {bmatrix} \boldupright {I} & \mathbb {E} \rvmJ _{\vs } & \mathbb {E} \rvmJ _{\mL } \\ \mathbb {E} \rvmJ _{\vs }^{\top } & \mathbb {E} \rvmJ _{\vs }^{\top } \rvmJ _{\vs } & \mathbb {E} \rvmJ _{\vs }^{\top } \rvmJ _{\mL } \\ \mathbb {E} \rvmJ _{\mL }^{\top } & \mathbb {E} \rvmJ _{\mL }^{\top } \rvmJ _{\vs } & \mathbb {E} \rvmJ _{\mL }^{\top } \rvmJ _{\mL } \end {bmatrix} \\ &= \begin {bmatrix} \boldupright {I} & & \\ & {\mathrm {diag}\left (\vphi \left (\vs \right )\right )}^2 & \\ & & \boldupright {I} \end {bmatrix}, \end {align*} which, conveniently, is a diagonal matrix. The maximal singular value of a block-diagonal matrix is the maximal singular value of each block. And since each block is diagonal with only positive entries, the largest element forms the maximal singular value. As we assume that \(\phi \) is 1-Lipchitz, the element of all blocks is lower-bounded by 0 and upper-bounded by 1. Therefore, the maximal singular value of the expected-squared Jacobian is bounded by 1.\end{proof}


==> main-pratendsmoothnesskey.tex <==


\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof]\phantomsection\label{proof:prAtEndiii}By the property of the Rayleigh quotients, for a symmetric matrix \(\mA \), its maximum eigenvalue is given in the variational form \[ \sup _{ \norm {\vx } \leq 1 } \vx ^{\top } \mH \vx = \sigma _{\mathrm {max}}\left (\mH \right ) \leq \sqrt { {\sigma _{\mathrm {max}}\left (\mH \right )}^2 } = \norm {\mH }_{2}, \] where \(\sigma _{\mathrm {max}}\left (\mA \right )\) is the maximal eigenvalue of \(\mA \). Notice the relationship with the \(\ell _2\)-operator norm. The inequality is strict only if all eigenvalues are negative. \par From the property above, \begin {alignat*}{2} {\lVert \mathbb {E} \rvmJ ^{\top } \rvmH \rvmJ \rVert }_2 &= \sup _{\norm {\vx }_2 \leq 1} \vx ^{\top } \left ( \mathbb {E}\rvmJ ^{\top } \rvmH \rvmJ \right ) \vx . \shortintertext {By reparameterizing as \(\rvvy = \rvmJ \vx \), } &= \sup _{\norm {\vx }_2 \leq 1} \mathbb {E} {\rvvy }^{\top } \rvmH \rvvy , \shortintertext {and the property of the \(\ell _2\)-operator norm,} &\leq \sup _{\norm {\vx }_2 \leq 1} \mathbb {E} \norm {\rvmH }_2 \norm {\rvvy }_2^2 = \sup _{\norm {\vx }_2 \leq 1} \mathbb {E} \norm {\rvmH }_2 \norm {\rvmJ \vx }_2^2. \shortintertext {From our assumption about the maximal eigenvalue of \(\mH \),} &\leq L \sup _{\norm {\vx }_2 \leq 1} \mathbb {E} \norm {\rvmJ \vx }_2^2, \shortintertext {denoting the \(\ell _2\) vector norm as a quadratic form as, } &= L \sup _{\norm {\vx }_2 \leq 1} \vx ^{\top } \left ( \mathbb {E} \rvmJ ^{\top } \rvmJ \right ) \vx , \shortintertext {again, by the property of the \(\ell _2\)-operator norm,} &\leq L {\lVert \mathbb {E} \rvmJ ^{\top } \rvmJ \rVert }_2 \sup _{\norm {\vx }_2 \leq 1} \norm {\vx }_2^2 \\ &= L {\lVert \mathbb {E} \rvmJ ^{\top } \rvmJ \rVert }_2. \end {alignat*}\end{proof}


==> thm_convex_proximal_sgd.tex <==

\begin{theoremEnd}[all end]{theorem}[Convergence of Proximal BBVI with Convex \(f\)]\label{thm:convex_proximal_sgd}
Let \(\ell\) be \(L_{\ell}\)-smooth and convex.
Then, for BBVI with a variational family satisfying \cref{assumption:variation_family}, the linear parameterization, and a nonincreasing stepsize sequence \(0 < \gamma_t \leq \frac{1}{2 L_f}\), the iterates satisfy
\[
  \mathbb{E} F\left( \bar{\vlambda}_T \right) - F \left( \vlambda^* \right)
  \leq
  \frac{
    \norm{\vlambda_0 - \vlambda^*}_2^2 + 2 \gamma_0 \left(F\left( \bar{\vlambda}_0 \right) - F \left( \vlambda^* \right)\right) 
  }{
    2 \left(1 -  4 \gamma_0 L_f\right) \sum^{T-1}_{t=0} \gamma_t
  }
  +
  \frac{
    2 \sigma^2 \sum^{T-1}_{t=0} \gamma_t^2
  }{
    \left( 1 - 4 \gamma_0 L_f \right) \sum^{T-1}_{t=0} \gamma_t
  },
\]
where, \(\bar{\vlambda}_T = \sum^{T-1}_{t=0} \vlambda_t / T \), \(\sigma^2\) is defined in \cref{thm:optimum_gradient_variance}, \(\vlambda^* \in \argmin_{\vlambda \in \Lambda} F\left(\vlambda\right)\), \(F^* = \inf_{\vlambda \in \Lambda} F\left(\vlambda\right)\).
\end{theoremEnd}
\vspace{-1ex}
\begin{proofEnd}
  Provided that
  \begin{enumerate}[label=\textbf{(A.\labelcref*{thm:convex_proximal_sgd}.\arabic*)},itemsep=-1ex]
    \item the energy \(f_{\mathrm{E}}\) is convex,~\label{eq:proximal_log_concave_cond1}
    \item the energy \(f_{\mathrm{E}}\) is \(L_f\)-smooth,~\label{eq:proximal_log_concave_cond7}
    \item the regularizer \(h\) is convex,~\label{eq:proximal_log_concave_cond2}
    \item the regularizer \(h\) is lower semi-continuous,~\label{eq:proximal_log_concave_cond3}
    \item the convex expected smoothness condition holds, and~\label{eq:proximal_log_concave_cond5}
    \item the gradient variance \(\sigma^2\) at the optimum is finite such that \(\sigma^2 < \infty\),~\label{eq:proximal_log_concave_cond6}
  \end{enumerate}
  the proof is identical to that of \citet[Theorem 11.5]{garrigos_handbook_2023}, which is based on the results of \citep[Theorem 3.3]{khaled_unified_2020}.

  In our setting,
  \begin{enumerate}[itemsep=-1ex]
    \item[\labelcref*{eq:proximal_log_concave_cond1}] is established by~\cref{thm:energy_convex}.
    \item[\labelcref*{eq:proximal_log_concave_cond7}] is established by~\cref{thm:energy_smooth}.
    \item[\labelcref*{eq:proximal_log_concave_cond2}] is trivially satisfied since \(h\) is the negative entropy,
    \item[\labelcref*{eq:proximal_log_concave_cond3}] is trivially satisfied since \(h\) is continuous, 
    \item[\labelcref*{eq:proximal_log_concave_cond5}] is established in \cref{thm:es_bregman},
    \item[\labelcref*{eq:proximal_log_concave_cond6}] is established in \cref{thm:optimum_gradient_variance}.
  \end{enumerate}
\end{proofEnd}


\begin{theoremEnd}[all end]{corollary}
  Let the assumptions of \cref{thm:convex_proximal_sgd} be satisfied.
  \begin{enumerate}[label=\textbf{(\roman*)}]
    \item With a fixed stepsize schedule such that \(0 < \gamma_t = \gamma < \frac{1}{4 L_f}\),\label{item:convex_sgd_fixed_stepsize}
\[
  \mathbb{E} F\left( \bar{\vlambda}_T \right) - F \left( \vlambda^* \right)
  \leq
  \frac{
    \norm{\vlambda_0 - \vlambda^*}_2^2 + 2 \gamma \left(F\left( \bar{\vlambda}_0 \right) - F \left( \vlambda^* \right)\right) 
  }{
    2 \left(1 -  4 \gamma L_f\right) \gamma T
  }
  +
  \frac{
    2 \sigma^2 \gamma
  }{
    \left( 1 - 4 \gamma L_f \right)
  }.
\]
    \item With a decreasing stepsize schedule \(\gamma_t  = \frac{\gamma_0}{\sqrt{t+1}} < \frac{1}{4 L_f}\),\label{item:convex_sgd_decreasing_stepsize}
\begin{align*}
  &\mathbb{E} F\left( \bar{\vlambda}_T \right) - F \left( \vlambda^* \right)
\\
  &\;\leq
\frac{1}{ \left(1 -  4 \gamma_0 L_f\right) \left(\sqrt{T} - \sqrt{2}\right) }
  \left(
  \frac{
    \norm{\vlambda_0 - \vlambda^*}_2^2
  }{
    4 \gamma_0 
  }
  + \frac{1}{2} \left(F\left( \bar{\vlambda}_0 \right) - F \left( \vlambda^* \right)\right) 
  +
  \sigma^2 \gamma_0 \log{T}
  \right),
\end{align*}
  \end{enumerate}
where \(\bar{\vlambda}_T = \sum^{T-1}_{t=0} \vlambda_t / T \), \(\sigma^2\) is defined in \cref{thm:optimum_gradient_variance}, \(\vlambda^* \in \argmin_{\vlambda \in \Lambda} F\left(\vlambda\right)\), \(F^* = \inf_{\vlambda \in \Lambda} F\left(\vlambda\right)\).
\end{theoremEnd}
\begin{proofEnd}
  \labelcref*{item:convex_sgd_fixed_stepsize} is trivial.

  \paragraph{Proof of \labelcref*{item:convex_sgd_decreasing_stepsize}}
  We use the well-known bounds on the cumulative stepsize
  \[
    \sum^{T}_{t=0} \gamma_t^2 \leq \gamma_0^2 \log{T}\quad\text{and}\quad
    \sum^{T}_{t=0} \gamma_t \geq 2 \gamma_0 \left(\sqrt{T} - \sqrt{2}\right).
  \]
  Plugging these bounds into \cref{thm:convex_proximal_sgd}, 
\begin{align*}
  &\mathbb{E} F\left( \bar{\vlambda}_T \right) - F \left( \vlambda^* \right)
  \\
  &\;\leq
  \frac{
    \norm{\vlambda_0 - \vlambda^*}_2^2 + 2 \gamma_0 \left(F\left( \bar{\vlambda}_0 \right) - F \left( \vlambda^* \right)\right) 
  }{
    2 \left(1 -  4 \gamma_0 L_f\right)  2 \gamma_0 \left(\sqrt{T} - \sqrt{2}\right)
  }
  +
  \frac{
    2 \sigma^2 \gamma_0^2 \log{T}
  }{
    \left( 1 - 4 \gamma_0 L_f \right) \; 2 \gamma_0 \left(\sqrt{T} - \sqrt{2}\right)
  }
  \\
  &\;=
  \frac{1}{ \left(1 -  4 \gamma_0 L_f\right) \left(\sqrt{T} - \sqrt{2}\right) }
  \left(
  \frac{
    \norm{\vlambda_0 - \vlambda^*}_2^2 + 2 \gamma_0 \left(F\left( \bar{\vlambda}_0 \right) - F \left( \vlambda^* \right)\right) 
  }{
    4 \gamma_0 
  }
  +
  \sigma^2 \gamma_0 \log{T}
  \right)
  \\
  &\;=
  \frac{1}{ \left(1 -  4 \gamma_0 L_f\right) \left(\sqrt{T} - \sqrt{2}\right) }
  \left(
  \frac{
    \norm{\vlambda_0 - \vlambda^*}_2^2
  }{
    4 \gamma_0 
  }
  + \frac{1}{2} \left(F\left( \bar{\vlambda}_0 \right) - F \left( \vlambda^* \right)\right) 
  +
  \sigma^2 \gamma_0 \log{T}
  \right)
\end{align*}

\end{proofEnd}


\begin{theoremEnd}[]{theorem}[Complexity of Proximal BBVI with Convex \(f\)]\label{thm:complexity_convex_proximal_sgd}
  Let \(f\) be \(L_f\)-smooth and convex.
  Then, for some \(0 < \epsilon \leq \nicefrac{\sigma^2}{L_f}\), BBVI with a variational family satisfying \cref{assumption:variation_family} and the linear parameterization generates the iterates \(\vlambda_1, \ldots, \vlambda_T\) that guarantee \(\mathbb{E} F\left(\bar{\vlambda}\right) - F^* \leq \epsilon\) if
  {%
\setlength{\belowdisplayskip}{.0ex} \setlength{\belowdisplayshortskip}{.0ex}
\setlength{\abovedisplayskip}{.5ex} \setlength{\abovedisplayshortskip}{.5ex}
\[
  \gamma = \frac{\epsilon}{8 \sigma^2}, \qquad
  T
  \geq
  16 \left(\norm{\vlambda_0 - \vlambda^*} + \frac{1}{4 L_f} \left(F\left(\vlambda_0\right) - F^*\right) \right) \frac{\sigma^2}{\epsilon^2},
\]
  }%
where \(\bar{\vlambda}_T = \sum^{T-1}_{t=0} \vlambda_t/T\), \(\sigma^2\) is defined in \cref{thm:optimum_gradient_variance}, \(\vlambda^* \in \argmin_{\vlambda \in \Lambda} F\left(\vlambda\right)\), and \(F^* = \inf_{\vlambda \in \Lambda} F\left(\vlambda\right)\).
\end{theoremEnd}
\vspace{-1ex}
\begin{proofEnd}
  This is a corollary of the full convergence guarantee~\cref{thm:convex_proximal_sgd} as shown by \citet[Corollary 11.8]{garrigos_handbook_2023}.
\end{proofEnd}



==> yian_notes.tex <==

\subsection{PL condition}
\begin{lemma}
\label{lem:grad_compute}
Consider the location-scale parametrization $\lambda=(m,C)$ with lower triagular matrix $C$. 
Denote $\diag(C)=\diag(\phi(s))$ and $\mathbf{1}_L\in R^{d\times d}$ as the strict lower triagular matrix with all one entries.
Then the gradient of the evidence lower bound $F(\lambda) = \E_{u\sim\varphi} f(t_\lambda(u)) - \log|C| + \mathrm{constant}$ is:
\[
\nabla_{\lambda} F(\lambda)
= \left( \E_{u\sim\varphi} \left[ \nabla f(t_\lambda(u)) u^\top - C^{-\top} \right] \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right) , \E_{u\sim\varphi} \nabla f(t_\lambda(u)) \right).
\]
\end{lemma}
Here, for $\xi=t_\lambda(u) = C u+m$, $f(\xi) = -\log p_{\xi}(\xi) = - \log \ell(x,\psi^{-1}(\xi)) - \log|J_{\psi^{-1}}(\xi)|$, where $\ell(x,z)$ is the posterior density of $z=\psi^{-1}(\xi)$.

% Assume that $\E_{\xi\sim q_{\lambda}} \left[ \nabla f(\xi) (\xi-m)^\top \right] \succeq \mathrm{I}$, and that $\phi$ is an increasing function, then we have convergence in $C$.
\begin{proof}
Setting the gradient equal to zero we have the conditions for the stationary points $C^*$ and $m^*$:
\[
\E_{u\sim\varphi} \nabla f(C^* u + m^*) = 0,
\]
and 
\[
\E_{u\sim\varphi} \left[ \nabla f(C^* u + m^*) u^\top - (C^*)^{-\top} \right] \circ \left( \diag(\phi'(s^*)) + \mathbf{1}_L \right) = 0.
\]
Note that $C^{-\top}$ is upper triangular.
Hence $C^{-\top} \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right) = \diag(C)^{-1} \circ \diag(\phi'(s)) = \diag(\phi'(s)) \diag(\phi(s))^{-1}$.
Using this fact, we obtain that 
\[
\E_{u\sim\varphi} \left[ \nabla f(C^* u + m^*) u^\top \right] \circ \left( \diag(\phi'(s^*)) + \mathbf{1}_L \right)
= \diag(\phi'(s^*)) \diag(\phi(s^*))^{-1}.
\]
...
So we must have $C^*$ is equal to the inverse of $Q_L$ if $f$ is a quadratic with matrix $Q$.

If function $f$ is convex, then
\begin{align}
\E_{u\sim\varphi} \left[ f(C u + m^*) - f(C^* u + m^*) \right] 
&\leq \E_{u\sim\varphi} \left\langle \nabla f(C u + m^*) , (C-C^*)u \right\rangle \nonumber\\
&= \mathrm{trace}\left( \E_{u\sim\varphi}\left[\nabla f(C u + m^*) u^\top\right] (C-C^*)^\top \right) \nonumber\\
&= \mathrm{trace}\left( \E_{u\sim\varphi}\left[ H(C,u,m^*) \cdot (C-C^*)u u^\top\right] (C-C^*)^\top \right),
\end{align}
where we denote $H(C,u,m) = \int_{0}^1 \nabla^2 f\left( (\tau C + (1-\tau) C^* ) u + m\right) {\rm d}\tau$ as the average Hessian of $f$.
On the other hand, we have
\begin{align*}
\nabla_C F(\lambda)
&= \E_{u\sim\varphi} \left[ \nabla f(C u + m) u^\top - C^{-\top} \right] \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right) \\
&= \E_{u\sim\varphi} \left[ H(C,u,m) \cdot (C-C^*) u u^\top - \left( C^{-\top} - (C^*)^{-\top} \right) \right] \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right)
\end{align*}

We first focus on the update in the lower triangular entries $C$ and assume for the moment that $\phi'(s)=1$: 
\begin{align*}
C_{t+1} = C_t - \eta_t \nabla_C F(\lambda)
= \E_{{u\sim\varphi}} \left[ \left( \mathbf{I} - \eta_t H(C_t,u,m) \right) \cdot (C_t-C^*) u u^\top \right] \circ \mathbf{1}_C + \diag(C_t)^{-1} - \diag(C^*)^{-1},
\end{align*}
where we have used the fact that $\E_{{u\sim\varphi}}[u u^\top]=\mathbf{I}$.
Therefore, 
\begin{align*}
\|C_{t+1}-C^*\|_F^2 
&= \left\| \E_{{u\sim\varphi}} \left[ \left( \mathbf{I} - \eta_t H(C,u,m) \right) \cdot (C-C^*) u u^\top \right] \circ \mathbf{1}_L \right\|_F^2 \\
&\leq \left\| \E_{{u\sim\varphi}} \left[ \left( \mathbf{I} - \eta_t H(C,u,m) \right) \cdot (C-C^*) u u^\top \right] \right\|_F^2.
\end{align*}
Assuming that $f$ is $m$-strongly convex, then $\left( \mathbf{I} - \eta_t H(C,u,m) \right)$ has a miximum eigenvalue of $1-\eta_t m$.
Therefore, 
\[\|C_{t+1}-C^*\|_F^2 \leq (1-\eta_t m) \|C_{t}-C^*\|_F^2. \]
% Using variable transformation, we have
% \[
% \E_{u\sim\varphi} \left[ \nabla f(t_\lambda(u)) u^\top \right]
% = \E_{\xi\sim q_\lambda} \left[ \nabla f(\xi) (\xi-m)^\top \right] C^{-\top}.
% \]
% Hence 
% \[
% \nabla_{\lambda_{C}} F(\lambda)
% = \left( \E_{\xi\sim q_\lambda} \left[ \nabla f(\xi) (\xi-m)^\top \right] - \mathrm{I} \right) C^{-\top} \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right) .
% \]
% Note that $C^{-\top}$ is upper triangular.
% Hence $C^{-\top} \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right) = \diag(C)^{-1} \circ \diag(\phi'(s)) = \diag(\phi'(s)) \diag(\phi(s))^{-1}$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:grad_compute}]
We first follow~\cite{kim_practical_2023} to compute the population gradient $\nabla_{\lambda} F(\lambda) = \E_{u\sim\varphi} \nabla_\lambda f(t_\lambda(u)) - \nabla_\lambda\log|C|$, where $\lambda=(m,C)$.

For
$\nabla_\lambda f(t_\lambda(u))
= \left[ \nabla_{\lambda_{m}} f(t_\lambda(u)), \nabla_{\lambda_{C}} f(t_\lambda(u)) \right]$, we first focus on $\nabla_{\lambda_{C}} f(t_\lambda(u))$:
\begin{align*}
\nabla_{\lambda_{C}} f(t_\lambda(u))
= \frac{\partial t_\lambda(u)}{\partial \lambda_{C}} \nabla f(t_\lambda(u)),
\end{align*}
where $\frac{\partial t_\lambda(u)}{\partial \lambda_{C}}$ is a third order tensor. For each individual entry $C_{ij}$, 
\[
\frac{\partial t_\lambda(u)}{\partial \lambda_{C_{ij}}} \nabla f(t_\lambda(u)) 
:= \left\langle \frac{\partial t_\lambda(u)}{\partial \lambda_{C_{ij}}}, \nabla f(t_\lambda(u))  \right\rangle.
\]
Then 
\begin{align*}
\frac{\partial t_\lambda(u)}{\partial \lambda_{C_{ij}}}
= \mathbf{e}_i u_j \frac{\partial C_{ij}}{\partial \lambda_{C_{ij}}},
\end{align*}
and that 
\[
\nabla_{\lambda_{C_{ij}}} f(t_\lambda(u))
= \nabla f_i(t_\lambda(u)) u_j \frac{\partial C_{ij}}{\partial \lambda_{C_{ij}}}.
\]
For the diagonal entries $\lambda_{C_{ii}} = s_i$ and $C_{ii}=\phi(s_i)$,
\[
\frac{\partial C_{ii}}{\partial \lambda_{C_{ii}}}
= \phi'(s_i).
\]
For the off-diagonal enties, $\lambda_{C_{ij}} = L_{ij}$,
\[
\frac{\partial C_{ij}}{\partial \lambda_{C_{ij}}} = 1.
\]
Hence 
\begin{align*}
\nabla_{\lambda_{C}} f(t_\lambda(u))
= \nabla f(t_\lambda(u)) u^\top \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right),
\end{align*}
where $\mathbf{1}_L\in R^{d\times d}$ denotes the strict lower triagular matrix with all ones, and $\circ$ denotes the Hardamard product.

We then compute 
\[
\nabla_{\lambda_{m}} f(t_\lambda(u))
= \frac{\partial t_\lambda(u)}{\partial \lambda_{m}} \nabla f(t_\lambda(u))
= \nabla f(t_\lambda(u)).
\]

We finally obtain that
\[
\nabla_\lambda\log|C|
= C^{-\top} \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right).
\]

Putting the results together, we arrive at the conclusion that 
\[
\nabla_{\lambda} F(\lambda)
= \E_{u\sim\varphi} \left[ \nabla f(t_\lambda(u)) u^\top - C^{-\top} \right] \circ \left( \diag(\phi'(s)) + \mathbf{1}_L \right) + \E_{u\sim\varphi} \nabla f(t_\lambda(u)).
\]
\end{proof}

